CORA: Benchmarks, Baselines, and Metrics as a Platform for Continual Reinforcement Learning Agents

Progress in continual reinforcement learning has been limited due to several barriers to entry: missing code, high compute requirements, and a lack of suitable benchmarks. In this work, we present CORA, a platform for Continual Reinforcement Learning Agents that provides benchmarks, baselines, and metrics in a single code package. The benchmarks we provide are designed to evaluate different aspects of the continual RL challenge, such as catastrophic forgetting, plasticity, ability to generalize, and sample-efficient learning. Three of the benchmarks utilize video game environments (Atari, Procgen, NetHack). The fourth benchmark, CHORES, consists of four different task sequences in a visually realistic home simulator, drawn from a diverse set of task and scene parameters. To compare continual RL methods on these benchmarks, we prepare three metrics in CORA: Continual Evaluation, Isolated Forgetting, and Zero-Shot Forward Transfer. Finally, CORA includes a set of performant, open-source baselines of existing algorithms for researchers to use and expand on. We release CORA and hope that the continual RL community can benefit from our contributions, to accelerate the development of new continual RL algorithms.

==> collas_template.tex <==
\clearpage

\newpage
\newpage
\section{Submission of conference papers to CoLLAs 2022}

CoLLAs requires electronic submissions, processed by
\href{https://openreview.net/}{https://openreview.net/}. See CoLLAs' website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}collasfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the ICLR format (which is inline with the NeurIPS format).
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to CoLLAs 2022 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the CoLLAs \LaTeX{} style files obtainable at the
CoLLAs website (\href{www.lifelong-ml.cc}{www.lifelong-ml.cc}). Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for CoLLAs and other conference information are available online at:
\begin{center}
   \href{http://www.lifelong-ml.cc/}{http://www.lifelong-ml.cc/}
\end{center}
The file \verb+collas2022_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your CoLLAs paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+collas2022_conference.sty+ and \verb+collas2022_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+collas2022_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 6.5~inches wide and
9~inches (54~picas) long. 
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author(s)'s name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\href{https://github.com/goodfeli/dlbook_notation/}{https://github.com/goodfeli/dlbook\_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.

\newpage 
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation \\ (\href{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps}{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\textbf{This should be only done in the camera ready version of the manuscript, not in the anonymized version submitted for review!}

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

\textbf{This should be only done in the camera ready version of the manuscript, not in the anonymized version submitted for review!}


\bibliography{collas2022_conference}
\bibliographystyle{collas2022_conference}

\appendix
\section{Appendix}
You may include other additional sections here.


==> images/atari/metrics/forgetting_tables.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
{} & {0-Space..} & {1-Krull} & {2-BeamR..} & {3-Hero} & {4-StarG..} & {5-MsPac..} & {Avg} \\
\hline
0-Space.. & \cellcolor{green!8} -2.0 & \cellcolor{red!13} 3.5 & \cellcolor{red!14} 3.6 & \cellcolor{red!14} 3.7 & \cellcolor{red!17} 4.3 & \cellcolor{red!15} 4.0 & \cellcolor{red!11} 2.8 \\
1-Krull & \cellcolor{red!23} 6.0 & \cellcolor{green!1} -0.5 & \cellcolor{red!20} 5.0 & \cellcolor{red!27} 7.0 & \cellcolor{red!23} 5.9 & \cellcolor{red!25} 6.3 & \cellcolor{red!19} 5.0 \\
2-BeamR.. & \cellcolor{red!33} 8.4 & \cellcolor{red!32} 8.2 & \cellcolor{green!0} -0.2 & \cellcolor{red!27} 6.8 & \cellcolor{red!33} 8.4 & \cellcolor{red!33} 8.5 & \cellcolor{red!26} 6.7 \\
3-Hero & \cellcolor{red!34} 8.5 & \cellcolor{red!34} 8.5 & \cellcolor{red!33} 8.3 & \cellcolor{red!0} 0.0 & \cellcolor{red!34} 8.5 & \cellcolor{red!34} 8.5 & \cellcolor{red!28} 7.1 \\
4-StarG.. & \cellcolor{red!26} 6.7 & \cellcolor{red!27} 6.8 & \cellcolor{red!26} 6.7 & \cellcolor{red!26} 6.7 & \cellcolor{green!5} -1.3 & \cellcolor{red!26} 6.6 & \cellcolor{red!21} 5.4 \\
5-MsPac.. & \cellcolor{red!21} 5.4 & \cellcolor{red!28} 7.2 & \cellcolor{red!25} 6.4 & \cellcolor{red!29} 7.3 & \cellcolor{red!26} 6.6 & \cellcolor{green!0} -0.2 & \cellcolor{red!21} 5.4 \\
\hline
Avg & \cellcolor{red!21} 5.5 & \cellcolor{red!22} 5.6 & \cellcolor{red!19} 5.0 & \cellcolor{red!21} 5.3 & \cellcolor{red!21} 5.4 & \cellcolor{red!22} 5.6 & \cellcolor{red!22} 5.6 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[EWC]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
{} & {0-Space..} & {1-Krull} & {2-BeamR..} & {3-Hero} & {4-StarG..} & {5-MsPac..} & {Avg} \\
\hline
0-Space.. & \cellcolor{red!7} 1.9 & \cellcolor{red!7} 1.8 & \cellcolor{red!6} 1.7 & \cellcolor{red!6} 1.7 & \cellcolor{red!7} 1.8 & \cellcolor{red!8} 2.2 & \cellcolor{red!7} 1.8 \\
1-Krull & \cellcolor{red!4} 1.0 & \cellcolor{red!2} 0.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!0} 0.2 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.2 & \cellcolor{red!3} 0.8 \\
2-BeamR.. & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.0 & \cellcolor{green!0} -0.1 & \cellcolor{red!2} 0.5 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.2 \\
3-Hero & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
4-StarG.. & \cellcolor{green!0} -0.1 & \cellcolor{green!1} -0.4 & \cellcolor{red!1} 0.3 & \cellcolor{green!0} -0.2 & \cellcolor{red!2} 0.6 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.1 \\
5-MsPac.. & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 0.8 & \cellcolor{red!4} 1.1 & \cellcolor{red!3} 1.0 & \cellcolor{red!4} 1.1 & \cellcolor{red!3} 0.9 & \cellcolor{red!3} 0.9 \\
\hline
Avg & \cellcolor{red!2} 0.7 & \cellcolor{red!2} 0.5 & \cellcolor{red!2} 0.6 & \cellcolor{red!1} 0.4 & \cellcolor{red!3} 0.8 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.7 \\
\hline
\end{tabular}
}




\subfloat[Online EWC]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
{} & {0-Space..} & {1-Krull} & {2-BeamR..} & {3-Hero} & {4-StarG..} & {5-MsPac..} & {Avg} \\
\hline
0-Space.. & \cellcolor{red!0} 0.0 & \cellcolor{red!21} 5.4 & \cellcolor{red!21} 5.3 & \cellcolor{red!19} 4.9 & \cellcolor{red!22} 5.5 & \cellcolor{red!22} 5.6 & \cellcolor{red!17} 4.5 \\
1-Krull & \cellcolor{red!24} 6.2 & \cellcolor{green!1} -0.3 & \cellcolor{red!17} 4.4 & \cellcolor{red!21} 5.3 & \cellcolor{red!30} 7.7 & \cellcolor{red!27} 6.8 & \cellcolor{red!19} 5.0 \\
2-BeamR.. & \cellcolor{red!13} 3.4 & \cellcolor{red!14} 3.6 & \cellcolor{green!4} -1.2 & \cellcolor{red!10} 2.5 & \cellcolor{red!12} 3.0 & \cellcolor{red!14} 3.6 & \cellcolor{red!9} 2.5 \\
3-Hero & \cellcolor{red!30} 7.7 & \cellcolor{red!30} 7.7 & \cellcolor{red!30} 7.7 & \cellcolor{green!1} -0.3 & \cellcolor{red!25} 6.3 & \cellcolor{red!30} 7.7 & \cellcolor{red!24} 6.1 \\
4-StarG.. & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.2 & \cellcolor{green!4} -1.1 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 \\
5-MsPac.. & \cellcolor{red!9} 2.5 & \cellcolor{red!16} 4.2 & \cellcolor{red!16} 4.2 & \cellcolor{red!15} 4.0 & \cellcolor{red!16} 4.2 & \cellcolor{green!6} -1.6 & \cellcolor{red!11} 2.9 \\
\hline
Avg & \cellcolor{red!13} 3.3 & \cellcolor{red!13} 3.5 & \cellcolor{red!13} 3.4 & \cellcolor{red!11} 2.8 & \cellcolor{red!17} 4.3 & \cellcolor{red!14} 3.7 & \cellcolor{red!15} 3.9 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
{} & {0-Space..} & {1-Krull} & {2-BeamR..} & {3-Hero} & {4-StarG..} & {5-MsPac..} & {Avg} \\
\hline
0-Space.. & \cellcolor{green!3} -1.0 & \cellcolor{red!16} 4.0 & \cellcolor{red!15} 3.9 & \cellcolor{red!13} 3.4 & \cellcolor{red!18} 4.7 & \cellcolor{red!19} 4.8 & \cellcolor{red!13} 3.3 \\
1-Krull & \cellcolor{red!19} 5.0 & \cellcolor{green!0} -0.1 & \cellcolor{red!19} 4.9 & \cellcolor{red!19} 4.8 & \cellcolor{red!22} 5.6 & \cellcolor{red!22} 5.5 & \cellcolor{red!17} 4.3 \\
2-BeamR.. & \cellcolor{red!26} 6.7 & \cellcolor{red!27} 6.8 & \cellcolor{green!1} -0.3 & \cellcolor{red!9} 2.3 & \cellcolor{red!27} 6.9 & \cellcolor{red!26} 6.7 & \cellcolor{red!19} 4.8 \\
3-Hero & \cellcolor{red!20} 5.1 & \cellcolor{red!20} 5.2 & \cellcolor{red!20} 5.2 & \cellcolor{green!13} -3.4 & \cellcolor{red!20} 5.2 & \cellcolor{red!20} 5.2 & \cellcolor{red!15} 3.8 \\
4-StarG.. & \cellcolor{red!28} 7.1 & \cellcolor{red!28} 7.1 & \cellcolor{red!28} 7.1 & \cellcolor{red!28} 7.1 & \cellcolor{green!5} -1.3 & \cellcolor{red!10} 2.7 & \cellcolor{red!19} 5.0 \\
5-MsPac.. & \cellcolor{red!21} 5.5 & \cellcolor{red!23} 5.8 & \cellcolor{red!19} 4.9 & \cellcolor{red!21} 5.4 & \cellcolor{red!22} 5.7 & \cellcolor{green!3} -0.9 & \cellcolor{red!17} 4.4 \\
\hline
Avg & \cellcolor{red!18} 4.7 & \cellcolor{red!19} 4.8 & \cellcolor{red!17} 4.3 & \cellcolor{red!13} 3.3 & \cellcolor{red!17} 4.5 & \cellcolor{red!16} 4.0 & \cellcolor{red!17} 4.4 \\
\hline
\end{tabular}
}




\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
{} & {0-Space..} & {1-Krull} & {2-BeamR..} & {3-Hero} & {4-StarG..} & {5-MsPac..} & {Avg} \\
\hline
0-Space.. & \cellcolor{green!5} -1.3 & \cellcolor{red!6} 1.7 & \cellcolor{red!5} 1.4 & \cellcolor{red!7} 1.8 & \cellcolor{red!9} 2.4 & \cellcolor{red!10} 2.6 & \cellcolor{red!5} 1.4 \\
1-Krull & \cellcolor{red!7} 1.8 & \cellcolor{green!2} -0.6 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.9 & \cellcolor{red!5} 1.4 \\
2-BeamR.. & \cellcolor{red!7} 2.0 & \cellcolor{red!10} 2.7 & \cellcolor{green!14} -3.7 & \cellcolor{red!2} 0.6 & \cellcolor{red!3} 0.8 & \cellcolor{red!6} 1.6 & \cellcolor{red!2} 0.6 \\
3-Hero & \cellcolor{red!3} 0.9 & \cellcolor{red!7} 1.9 & \cellcolor{red!3} 0.9 & \cellcolor{green!2} -0.6 & \cellcolor{red!0} 0.1 & \cellcolor{red!4} 1.1 & \cellcolor{red!2} 0.7 \\
4-StarG.. & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.2 & \cellcolor{green!16} -4.1 & \cellcolor{green!2} -0.5 & \cellcolor{red!2} 0.7 \\
5-MsPac.. & \cellcolor{red!0} 0.2 & \cellcolor{red!7} 1.9 & \cellcolor{red!4} 1.2 & \cellcolor{red!5} 1.3 & \cellcolor{red!4} 1.2 & \cellcolor{green!6} -1.6 & \cellcolor{red!2} 0.7 \\
\hline
Avg & \cellcolor{red!3} 0.9 & \cellcolor{red!6} 1.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!4} 1.2 & \cellcolor{red!1} 0.4 & \cellcolor{red!3} 0.8 & \cellcolor{red!4} 1.1 \\
\hline
\end{tabular}
}


==> images/atari/metrics/forgetting_tables_old.tex <==
\subfloat[IMPALA]{
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} \\
\hline
0-Space... & \cellcolor{white!20} -- & \cellcolor{red!20} 618.6 & \cellcolor{red!20} 596.0 & \cellcolor{red!20} 551.2 & \cellcolor{red!20} 723.4 & \cellcolor{red!20} 678.9 & \cellcolor{green!20} -330.9 & \cellcolor{red!20} 523.0 & \cellcolor{red!20} 592.3 & \cellcolor{red!20} 652.4 & \cellcolor{red!20} 673.9 & \cellcolor{red!20} 626.3 \\
1-Krull & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 5709.6 & \cellcolor{red!20} 7107.4 & \cellcolor{red!20} 5698.0 & \cellcolor{red!20} 6714.3 & \cellcolor{red!20} 6066.8 & \cellcolor{green!20} -464.5 & \cellcolor{red!20} 4475.4 & \cellcolor{red!20} 7010.2 & \cellcolor{red!20} 6275.4 & \cellcolor{red!20} 6133.7 \\
2-BeamR... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 6135.6 & \cellcolor{red!20} 8183.2 & \cellcolor{red!20} 8178.9 & \cellcolor{red!20} 8084.5 & \cellcolor{red!20} 7958.8 & \cellcolor{green!20} -209.5 & \cellcolor{red!20} 7054.6 & \cellcolor{red!20} 8118.4 & \cellcolor{red!20} 8157.3 \\
3-Hero & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 19592.0 & \cellcolor{red!20} 19592.0 & \cellcolor{red!20} 19591.7 & \cellcolor{red!20} 19592.0 & \cellcolor{red!20} 19082.8 & \cellcolor{red!20} 105.2 & \cellcolor{red!20} 19577.5 & \cellcolor{red!20} 19592.0 \\
4-StarG... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 71301.0 & \cellcolor{red!20} 71991.2 & \cellcolor{red!20} 72125.5 & \cellcolor{red!20} 71888.5 & \cellcolor{red!20} 71873.3 & \cellcolor{green!20} -13692.2 & \cellcolor{red!20} 68942.1 \\
5-MsPac... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1400.1 & \cellcolor{red!20} 1862.4 & \cellcolor{red!20} 1666.8 & \cellcolor{red!20} 1893.7 & \cellcolor{red!20} 1720.4 & \cellcolor{green!20} -56.0 \\
\hline
\end{tabular}
}

\subfloat[EWC]{
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} \\
\hline
0-Space... & \cellcolor{white!20} -- & \cellcolor{red!20} 308.7 & \cellcolor{red!20} 264.2 & \cellcolor{red!20} 268.4 & \cellcolor{red!20} 275.9 & \cellcolor{red!20} 324.0 & \cellcolor{red!20} 264.3 & \cellcolor{red!20} 177.3 & \cellcolor{red!20} 202.0 & \cellcolor{red!20} 194.5 & \cellcolor{red!20} 203.0 & \cellcolor{red!20} 265.5 \\
1-Krull & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 272.1 & \cellcolor{red!20} 51.3 & \cellcolor{red!20} 890.9 & \cellcolor{red!20} 862.4 & \cellcolor{red!20} 451.4 & \cellcolor{red!20} 243.8 & \cellcolor{red!20} 204.9 & \cellcolor{red!20} 85.9 & \cellcolor{red!20} 73.4 & \cellcolor{red!20} 166.5 \\
2-BeamR... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -25.9 & \cellcolor{red!20} 59.0 & \cellcolor{red!20} 18.1 & \cellcolor{red!20} 26.5 & \cellcolor{red!20} 21.7 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 15.7 & \cellcolor{red!20} 24.9 & \cellcolor{green!20} -3.4 \\
3-Hero & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 \\
4-StarG... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -25.0 & \cellcolor{green!20} -6.8 & \cellcolor{green!20} -33.2 & \cellcolor{red!20} 22.5 & \cellcolor{green!20} -16.9 & \cellcolor{red!20} 54.6 & \cellcolor{red!20} 82.5 \\
5-MsPac... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 58.8 & \cellcolor{red!20} 66.4 & \cellcolor{red!20} 88.9 & \cellcolor{red!20} 80.0 & \cellcolor{red!20} 85.6 & \cellcolor{red!20} 75.4 \\
\hline
\end{tabular}
}

\subfloat[ONLINE EWC]{
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} \\
\hline
0-Space... & \cellcolor{white!20} -- & \cellcolor{red!20} 586.3 & \cellcolor{red!20} 514.3 & \cellcolor{red!20} 540.3 & \cellcolor{red!20} 602.3 & \cellcolor{red!20} 583.9 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 486.7 & \cellcolor{red!20} 541.4 & \cellcolor{red!20} 450.1 & \cellcolor{red!20} 507.8 & \cellcolor{red!20} 533.7 \\
1-Krull & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 4348.1 & \cellcolor{red!20} 4766.8 & \cellcolor{red!20} 5998.0 & \cellcolor{red!20} 5593.2 & \cellcolor{red!20} 4729.3 & \cellcolor{green!20} -268.0 & \cellcolor{red!20} 2335.9 & \cellcolor{red!20} 3395.2 & \cellcolor{red!20} 5789.4 & \cellcolor{red!20} 4821.1 \\
2-BeamR... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 839.2 & \cellcolor{red!20} 993.1 & \cellcolor{red!20} 1173.9 & \cellcolor{red!20} 1090.7 & \cellcolor{red!20} 1172.0 & \cellcolor{green!20} -385.6 & \cellcolor{red!20} 807.3 & \cellcolor{red!20} 985.6 & \cellcolor{red!20} 1171.0 \\
3-Hero & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 9742.8 & \cellcolor{red!20} 12517.3 & \cellcolor{red!20} 12517.3 & \cellcolor{red!20} 12517.3 & \cellcolor{red!20} 12494.3 & \cellcolor{green!20} -423.5 & \cellcolor{red!20} 10611.5 & \cellcolor{red!20} 12517.3 \\
4-StarG... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 793.0 & \cellcolor{red!20} 1197.2 & \cellcolor{red!20} 1103.6 & \cellcolor{red!20} 1203.1 & \cellcolor{red!20} 1064.6 & \cellcolor{green!20} -5732.2 & \cellcolor{green!20} -1732.8 \\
5-MsPac... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 852.1 & \cellcolor{red!20} 1447.5 & \cellcolor{red!20} 1454.2 & \cellcolor{red!20} 1367.2 & \cellcolor{red!20} 1442.4 & \cellcolor{green!20} -546.0 \\
\hline
\end{tabular}
}

\subfloat[P\&C]{
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} \\
\hline
0-Space... & \cellcolor{white!20} -- & \cellcolor{red!20} 648.6 & \cellcolor{red!20} 546.8 & \cellcolor{red!20} 460.0 & \cellcolor{red!20} 686.2 & \cellcolor{red!20} 675.9 & \cellcolor{green!20} -135.4 & \cellcolor{red!20} 487.5 & \cellcolor{red!20} 559.4 & \cellcolor{red!20} 491.8 & \cellcolor{red!20} 627.6 & \cellcolor{red!20} 680.5 \\
1-Krull & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 5426.4 & \cellcolor{red!20} 5532.5 & \cellcolor{red!20} 5851.5 & \cellcolor{red!20} 5925.6 & \cellcolor{red!20} 5494.0 & \cellcolor{green!20} -64.2 & \cellcolor{red!20} 5434.3 & \cellcolor{red!20} 5068.9 & \cellcolor{red!20} 6371.3 & \cellcolor{red!20} 6199.2 \\
2-BeamR... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1396.7 & \cellcolor{red!20} 4051.5 & \cellcolor{red!20} 3978.8 & \cellcolor{red!20} 3937.7 & \cellcolor{red!20} 3996.4 & \cellcolor{green!20} -184.0 & \cellcolor{red!20} 1344.8 & \cellcolor{red!20} 4067.6 & \cellcolor{red!20} 3945.4 \\
3-Hero & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 11450.7 & \cellcolor{red!20} 11450.7 & \cellcolor{red!20} 11266.9 & \cellcolor{red!20} 11450.7 & \cellcolor{red!20} 11450.7 & \cellcolor{green!20} -7501.0 & \cellcolor{red!20} 11437.5 & \cellcolor{red!20} 11433.3 \\
4-StarG... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 27044.0 & \cellcolor{red!20} 40435.3 & \cellcolor{red!20} 40500.1 & \cellcolor{red!20} 40529.5 & \cellcolor{red!20} 40443.0 & \cellcolor{green!20} -7360.6 & \cellcolor{red!20} 3864.5 \\
5-MsPac... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1041.6 & \cellcolor{red!20} 1097.7 & \cellcolor{red!20} 937.6 & \cellcolor{red!20} 1034.7 & \cellcolor{red!20} 1083.6 & \cellcolor{green!20} -169.4 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} & {0-Space...} & {1-Krull} & {2-BeamR...} & {3-Hero} & {4-StarG...} & {5-MsPac...} \\
\hline
0-Space... & \cellcolor{white!20} -- & \cellcolor{red!20} 1401.5 & \cellcolor{red!20} 1123.7 & \cellcolor{red!20} 1302.6 & \cellcolor{red!20} 1348.6 & \cellcolor{red!20} 1429.2 & \cellcolor{green!20} -502.1 & \cellcolor{green!20} -98.3 & \cellcolor{green!20} -25.4 & \cellcolor{red!20} 71.7 & \cellcolor{red!20} 482.8 & \cellcolor{red!20} 600.1 \\
1-Krull & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 2165.6 & \cellcolor{red!20} 2053.5 & \cellcolor{red!20} 1833.5 & \cellcolor{red!20} 2199.0 & \cellcolor{red!20} 2074.5 & \cellcolor{green!20} -683.9 & \cellcolor{red!20} 1997.5 & \cellcolor{red!20} 2041.9 & \cellcolor{red!20} 2352.0 & \cellcolor{red!20} 2268.2 \\
2-BeamR... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 927.6 & \cellcolor{red!20} 464.3 & \cellcolor{red!20} 1182.7 & \cellcolor{red!20} 1103.6 & \cellcolor{red!20} 1496.5 & \cellcolor{green!20} -2084.6 & \cellcolor{green!20} -208.3 & \cellcolor{red!20} 406.6 & \cellcolor{red!20} 584.2 \\
3-Hero & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 704.5 & \cellcolor{red!20} 7172.1 & \cellcolor{red!20} 3421.1 & \cellcolor{red!20} 6931.0 & \cellcolor{red!20} 3396.9 & \cellcolor{green!20} -2299.6 & \cellcolor{green!20} -52.7 & \cellcolor{red!20} 948.3 \\
4-StarG... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 11231.8 & \cellcolor{red!20} 16735.3 & \cellcolor{red!20} 17259.9 & \cellcolor{red!20} 17223.8 & \cellcolor{red!20} 17639.3 & \cellcolor{green!20} -32751.8 & \cellcolor{green!20} -19924.0 \\
5-MsPac... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 87.6 & \cellcolor{red!20} 914.1 & \cellcolor{red!20} 589.6 & \cellcolor{red!20} 619.1 & \cellcolor{red!20} 556.5 & \cellcolor{green!20} -770.5 \\
\hline
\end{tabular}
}

==> images/atari/metrics/transfer_tables.tex <==

\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Space.. & 1-Krull & 2-BeamR.. & 3-Hero & 4-StarG.. & 5-MsPac.. & Avg \\
\hline
0-Space.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Krull & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
2-BeamR.. & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
3-Hero & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
4-StarG.. & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
5-MsPac.. & \cellcolor{green!2} 0.6 & \cellcolor{red!1} -0.4 & \cellcolor{green!2} 0.7 & \cellcolor{red!3} -0.8 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
Avg & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.3 & \cellcolor{red!1} -0.4 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
\end{tabular}
}
\subfloat[EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Space.. & 1-Krull & 2-BeamR.. & 3-Hero & 4-StarG.. & 5-MsPac.. & Avg \\
\hline
0-Space.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Krull & \cellcolor{green!7} 1.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.9 \\
2-BeamR.. & \cellcolor{green!0} 0.2 & \cellcolor{red!10} -2.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!5} -1.3 \\
3-Hero & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
4-StarG.. & \cellcolor{green!13} 3.3 & \cellcolor{red!6} -1.7 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
5-MsPac.. & \cellcolor{green!6} 1.6 & \cellcolor{red!5} -1.4 & \cellcolor{green!3} 0.8 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
\hline
Avg & \cellcolor{green!5} 1.4 & \cellcolor{red!5} -1.5 & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.1 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
\end{tabular}
}

\subfloat[Online EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Space.. & 1-Krull & 2-BeamR.. & 3-Hero & 4-StarG.. & 5-MsPac.. & Avg \\
\hline
0-Space.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Krull & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
2-BeamR.. & \cellcolor{green!0} 0.1 & \cellcolor{red!2} -0.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.3 \\
3-Hero & \cellcolor{green!1} 0.3 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
4-StarG.. & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
5-MsPac.. & \cellcolor{green!3} 0.8 & \cellcolor{red!3} -0.9 & \cellcolor{green!0} 0.2 & \cellcolor{green!1} 0.4 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
\hline
Avg & \cellcolor{green!0} 0.2 & \cellcolor{red!1} -0.5 & \cellcolor{green!0} 0.1 & \cellcolor{green!0} 0.2 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
\end{tabular}
}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Space.. & 1-Krull & 2-BeamR.. & 3-Hero & 4-StarG.. & 5-MsPac.. & Avg \\
\hline
0-Space.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Krull & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
2-BeamR.. & \cellcolor{green!1} 0.3 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
3-Hero & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
4-StarG.. & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
5-MsPac.. & \cellcolor{red!2} -0.7 & \cellcolor{red!1} -0.4 & \cellcolor{green!6} 1.6 & \cellcolor{red!3} -1.0 & \cellcolor{red!2} -0.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
\hline
Avg & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.1 & \cellcolor{green!2} 0.5 & \cellcolor{red!1} -0.5 & \cellcolor{red!2} -0.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Space.. & 1-Krull & 2-BeamR.. & 3-Hero & 4-StarG.. & 5-MsPac.. & Avg \\
\hline
0-Space.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Krull & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.3 \\
2-BeamR.. & \cellcolor{red!1} -0.3 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
3-Hero & \cellcolor{red!0} 0.0 & \cellcolor{green!0} 0.0 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
4-StarG.. & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
5-MsPac.. & \cellcolor{green!1} 0.5 & \cellcolor{red!1} -0.3 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
\hline` 
Avg & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
\hline
\end{tabular}
}


==> images/atari/metrics/transfer_tables_old.tex <==
\subfloat[IMPALA]{
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-SpaceInvaders (C0)} & {1-Krull (C0)} & {2-BeamRider (C0)} & {3-Hero (C0)} & {4-StarGunner (C0)} & {5-MsPacman (C0)} \\
\hline
0-SpaceInvaders & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Krull & \cellcolor{green!20} 55.7 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-BeamRider & \cellcolor{green!20} 164.2 & \cellcolor{green!20} 177.7 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Hero & \cellcolor{green!20} 4.3 & \cellcolor{white!20} 0.0 & \cellcolor{green!20} 501.8 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-StarGunner & \cellcolor{green!20} 303.5 & \cellcolor{green!20} 26.7 & \cellcolor{green!20} 247.6 & \cellcolor{green!20} 264.8 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-MsPacman & \cellcolor{green!20} 168.0 & \cellcolor{green!20} 73.8 & \cellcolor{green!20} 245.0 & \cellcolor{green!20} 46.9 & \cellcolor{green!20} 88.7 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[EWC]{
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-SpaceInvaders (C0)} & {1-Krull (C0)} & {2-BeamRider (C0)} & {3-Hero (C0)} & {4-StarGunner (C0)} & {5-MsPacman (C0)} \\
\hline
0-SpaceInvaders & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Krull & \cellcolor{green!20} 832.6 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-BeamRider & \cellcolor{green!20} 17.3 & \cellcolor{red!20} -212.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Hero & \cellcolor{green!20} 3.9 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-StarGunner & \cellcolor{green!20} 283.6 & \cellcolor{green!20} 136.6 & \cellcolor{green!20} 129.2 & \cellcolor{green!20} 153.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-MsPacman & \cellcolor{green!20} 130.3 & \cellcolor{green!20} 18.2 & \cellcolor{green!20} 79.8 & \cellcolor{green!20} 65.5 & \cellcolor{green!20} 73.0 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[ONLINE EWC]{
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-SpaceInvaders (C0)} & {1-Krull (C0)} & {2-BeamRider (C0)} & {3-Hero (C0)} & {4-StarGunner (C0)} & {5-MsPacman (C0)} \\
\hline
0-SpaceInvaders & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Krull & \cellcolor{red!20} -159.5 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-BeamRider & \cellcolor{green!20} 34.1 & \cellcolor{red!20} -208.9 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Hero & \cellcolor{green!20} 439.4 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-StarGunner & \cellcolor{green!20} 156.6 & \cellcolor{green!20} 118.6 & \cellcolor{green!20} 197.1 & \cellcolor{green!20} 150.9 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-MsPacman & \cellcolor{green!20} 288.9 & \cellcolor{red!20} -25.9 & \cellcolor{green!20} 48.5 & \cellcolor{green!20} 175.7 & \cellcolor{green!20} 52.7 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[P\&C]{
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-SpaceInvaders (C0)} & {1-Krull (C0)} & {2-BeamRider (C0)} & {3-Hero (C0)} & {4-StarGunner (C0)} & {5-MsPacman (C0)} \\
\hline
0-SpaceInvaders & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Krull & \cellcolor{green!20} 409.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-BeamRider & \cellcolor{green!20} 153.8 & \cellcolor{green!20} 177.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Hero & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-StarGunner & \cellcolor{red!20} -16.9 & \cellcolor{green!20} 68.5 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 120.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-MsPacman & \cellcolor{red!20} -132.3 & \cellcolor{red!20} -213.0 & \cellcolor{green!20} 89.3 & \cellcolor{red!20} -96.9 & \cellcolor{red!20} -217.7 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-SpaceInvaders (C0)} & {1-Krull (C0)} & {2-BeamRider (C0)} & {3-Hero (C0)} & {4-StarGunner (C0)} & {5-MsPacman (C0)} \\
\hline
0-SpaceInvaders & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Krull & \cellcolor{green!20} 309.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-BeamRider & \cellcolor{red!20} -177.6 & \cellcolor{red!20} -63.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Hero & \cellcolor{white!20} 0.0 & \cellcolor{green!20} 14.6 & \cellcolor{green!20} 319.2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-StarGunner & \cellcolor{green!20} 166.0 & \cellcolor{green!20} 131.1 & \cellcolor{green!20} 249.7 & \cellcolor{green!20} 294.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-MsPacman & \cellcolor{green!20} 218.4 & \cellcolor{green!20} 93.6 & \cellcolor{green!20} 224.5 & \cellcolor{green!20} 163.2 & \cellcolor{green!20} 100.7 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

==> images/chores/metrics/multi_traj_forgetting.tex <==
\subfloat[EWC]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R19, Cu..} & {R13, Po..} & {R02, Le..} & {Avg} \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!7} 1.9 & \cellcolor{red!6} 1.7 & \cellcolor{red!7} 1.8 \\
R13, Po.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!2} 0.5 & \cellcolor{red!2} 0.5 \\
R02, Le.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{red!7} 1.9 & \cellcolor{red!4} 1.1 & \cellcolor{red!5} 1.4 \\
\hline
\end{tabular}
}
\hspace{1em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R19, Cu..} & {R13, Po..} & {R02, Le..} & {Avg} \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 \\
R13, Po.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 \\
R02, Le.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 \\
\hline
\end{tabular}
}
\hspace{1em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R19, Cu..} & {R13, Po..} & {R02, Le..} & {Avg} \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!5} 1.3 & \cellcolor{green!0} -0.0 & \cellcolor{red!2} 0.6 \\
R13, Po.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} -0.9 & \cellcolor{green!3} -0.9 \\
R02, Le.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{red!5} 1.3 & \cellcolor{green!1} -0.5 & \cellcolor{red!0} 0.1 \\
\hline
\end{tabular}
}


==> images/chores/metrics/multi_traj_transfer.tex <==

\subfloat[EWC]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R19, Cu.. & R13, Po.. & R02, Le.. & Avg \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R13, Po.. & \cellcolor{red!13} -3.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!13} -3.5 \\
R02, Le.. & \cellcolor{red!25} -6.3 & \cellcolor{red!9} -2.3 & \cellcolor{red!0} -- & \cellcolor{red!17} -4.3 \\
\hline
Avg & \cellcolor{red!19} -4.9 & \cellcolor{red!9} -2.3 & \cellcolor{red!0} -- & \cellcolor{red!16} -4.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R19, Cu.. & R13, Po.. & R02, Le.. & Avg \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R13, Po.. & \cellcolor{green!3} 0.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.9 \\
R02, Le.. & \cellcolor{green!0} 0.0 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
\hline
Avg & \cellcolor{green!1} 0.4 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R19, Cu.. & R13, Po.. & R02, Le.. & Avg \\
\hline
R19, Cu.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R13, Po.. & \cellcolor{red!16} -4.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!16} -4.1 \\
R02, Le.. & \cellcolor{red!39} -9.8 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!19} -5.0 \\
\hline
Avg & \cellcolor{red!27} -7.0 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!18} -4.7 \\
\hline
\end{tabular}
}



==> images/chores/metrics/vary_envs_forgetting.tex <==

\subfloat[EWC]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R402} & {R419} & {R423} & {Avg} \\
\hline
R402 & \cellcolor{red!5} 1.4 & \cellcolor{red!9} 2.4 & \cellcolor{red!5} 1.4 & \cellcolor{red!6} 1.7 \\
R419 & \cellcolor{green!13} -3.5 & \cellcolor{red!0} 0.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!4} -1.2 \\
R423 & \cellcolor{green!0} -0.1 & \cellcolor{red!13} 3.3 & \cellcolor{red!13} 3.4 & \cellcolor{red!8} 2.2 \\
\hline
Avg & \cellcolor{green!2} -0.7 & \cellcolor{red!7} 1.9 & \cellcolor{red!6} 1.6 & \cellcolor{red!3} 1.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R402} & {R419} & {R423} & {Avg} \\
\hline
R402 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
R419 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
R423 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
\hline
Avg & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {R402} & {R419} & {R423} & {Avg} \\
\hline
R402 & \cellcolor{green!6} -1.6 & \cellcolor{red!14} 3.6 & \cellcolor{red!11} 2.8 & \cellcolor{red!6} 1.6 \\
R419 & \cellcolor{green!13} -3.3 & \cellcolor{green!26} -6.7 & \cellcolor{green!26} -6.6 & \cellcolor{green!22} -5.5 \\
R423 & \cellcolor{green!2} -0.5 & \cellcolor{green!13} -3.3 & \cellcolor{green!12} -3.2 & \cellcolor{green!9} -2.4 \\
\hline
Avg & \cellcolor{green!7} -1.8 & \cellcolor{green!8} -2.2 & \cellcolor{green!9} -2.3 & \cellcolor{green!6} -1.6 \\
\hline
\end{tabular}
}



==> images/chores/metrics/vary_envs_transfer.tex <==

\subfloat[EWC]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R402 & R419 & R423 & Avg \\
\hline
R402 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R419 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
R423 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
\hline
Avg & \cellcolor{red!0} -0.1 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R402 & R419 & R423 & Avg \\
\hline
R402 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R419 & \cellcolor{green!19} 4.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!19} 4.8 \\
R423 & \cellcolor{green!19} 4.8 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!9} 2.4 \\
\hline
Avg & \cellcolor{green!19} 4.8 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!12} 3.2 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & R402 & R419 & R423 & Avg \\
\hline
R402 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
R419 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
R423 & \cellcolor{red!8} -2.0 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{red!6} -1.7 \\
\hline
Avg & \cellcolor{red!4} -1.0 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{red!4} -1.1 \\
\hline
\end{tabular}
}

==> images/chores/metrics/vary_objects_forgetting.tex <==
\subfloat[EWC]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Fork} & {Knife} & {Spoon} & {Avg} \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{red!13} 3.4 & \cellcolor{red!0} 0.2 & \cellcolor{red!7} 1.8 \\
Knife & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!12} -3.2 & \cellcolor{green!12} -3.2 \\
Spoon & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{red!13} 3.4 & \cellcolor{green!6} -1.5 & \cellcolor{red!0} 0.1 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Fork} & {Knife} & {Spoon} & {Avg} \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{green!0} -0.0 & \cellcolor{red!12} 3.0 & \cellcolor{red!6} 1.5 \\
Knife & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!11} 3.0 & \cellcolor{red!11} 3.0 \\
Spoon & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{green!0} -0.0 & \cellcolor{red!12} 3.0 & \cellcolor{red!8} 2.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Fork} & {Knife} & {Spoon} & {Avg} \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{red!26} 6.7 & \cellcolor{red!28} 7.1 & \cellcolor{red!27} 6.9 \\
Knife & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!11} 2.9 & \cellcolor{red!11} 2.9 \\
Spoon & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
\hline
Avg & \cellcolor{red!0} -- & \cellcolor{red!26} 6.7 & \cellcolor{red!20} 5.0 & \cellcolor{red!22} 5.6 \\
\hline
\end{tabular}
}

==> images/chores/metrics/vary_objects_transfer.tex <==

\subfloat[EWC]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Fork & Knife & Spoon & Avg \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Knife & \cellcolor{green!25} 6.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!25} 6.4 \\
Spoon & \cellcolor{green!27} 6.9 & \cellcolor{red!21} -5.3 & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
\hline
Avg & \cellcolor{green!26} 6.6 & \cellcolor{red!21} -5.3 & \cellcolor{red!0} -- & \cellcolor{green!10} 2.6 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Fork & Knife & Spoon & Avg \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Knife & \cellcolor{green!37} 9.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!37} 9.3 \\
Spoon & \cellcolor{green!32} 8.2 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{green!13} 3.4 \\
\hline
Avg & \cellcolor{green!34} 8.7 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{green!21} 5.4 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Fork & Knife & Spoon & Avg \\
\hline
Fork & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Knife & \cellcolor{red!37} -9.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!37} -9.4 \\
Spoon & \cellcolor{red!25} -6.4 & \cellcolor{green!7} 1.8 & \cellcolor{red!0} -- & \cellcolor{red!9} -2.3 \\
\hline
Avg & \cellcolor{red!31} -7.9 & \cellcolor{green!7} 1.8 & \cellcolor{red!0} -- & \cellcolor{red!18} -4.6 \\
\hline
\end{tabular}
}



==> images/chores/metrics/vary_tasks_forgetting.tex <==
\subfloat[EWC]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Hang TP} & {Counter} & {Cabinet} & {Avg} \\
\hline
Hang TP & \cellcolor{green!25} -6.5 & \cellcolor{green!19} -4.9 & \cellcolor{green!14} -3.6 & \cellcolor{green!19} -5.0 \\
Counter & \cellcolor{red!28} 7.2 & \cellcolor{red!9} 2.4 & \cellcolor{red!16} 4.1 & \cellcolor{red!18} 4.6 \\
Cabinet & \cellcolor{red!20} 5.2 & \cellcolor{green!7} -1.9 & \cellcolor{green!23} -6.0 & \cellcolor{green!3} -0.9 \\
\hline
Avg & \cellcolor{red!7} 2.0 & \cellcolor{green!5} -1.4 & \cellcolor{green!7} -1.8 & \cellcolor{green!2} -0.7 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Hang TP} & {Counter} & {Cabinet} & {Avg} \\
\hline
Hang TP & \cellcolor{green!12} -3.2 & \cellcolor{green!6} -1.5 & \cellcolor{green!12} -3.2 & \cellcolor{green!10} -2.6 \\
Counter & \cellcolor{green!13} -3.5 & \cellcolor{green!13} -3.5 & \cellcolor{green!13} -3.5 & \cellcolor{green!13} -3.5 \\
Cabinet & \cellcolor{red!0} 0.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.0 \\
\hline
Avg & \cellcolor{green!8} -2.2 & \cellcolor{green!6} -1.7 & \cellcolor{green!8} -2.2 & \cellcolor{green!8} -2.2 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lll|l|}
\hline
{} & {Hang TP} & {Counter} & {Cabinet} & {Avg} \\
\hline
Hang TP & \cellcolor{green!20} -5.2 & \cellcolor{red!18} 4.6 & \cellcolor{red!14} 3.7 & \cellcolor{red!4} 1.0 \\
Counter & \cellcolor{red!1} 0.3 & \cellcolor{green!24} -6.1 & \cellcolor{green!3} -1.0 & \cellcolor{green!9} -2.3 \\
Cabinet & \cellcolor{red!11} 2.9 & \cellcolor{red!13} 3.4 & \cellcolor{green!8} -2.1 & \cellcolor{red!5} 1.4 \\
\hline
Avg & \cellcolor{green!2} -0.7 & \cellcolor{red!2} 0.6 & \cellcolor{red!0} 0.2 & \cellcolor{red!2} 0.6 \\
\hline
\end{tabular}
}

==> images/chores/metrics/vary_tasks_transfer.tex <==

\subfloat[EWC]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Hang TP & Counter & Cabinet & Avg \\
\hline
Hang TP & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Counter & \cellcolor{red!26} -6.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!26} -6.7 \\
Cabinet & \cellcolor{red!25} -6.3 & \cellcolor{green!4} 1.1 & \cellcolor{red!0} -- & \cellcolor{red!10} -2.6 \\
\hline
Avg & \cellcolor{red!26} -6.5 & \cellcolor{green!4} 1.1 & \cellcolor{red!0} -- & \cellcolor{red!15} -4.0 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Hang TP & Counter & Cabinet & Avg \\
\hline
Hang TP & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Counter & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
Cabinet & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
Avg & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llH|l|}
\hline
 & Hang TP & Counter & Cabinet & Avg \\
\hline
Hang TP & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
Counter & \cellcolor{red!29} -7.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!29} -7.5 \\
Cabinet & \cellcolor{red!8} -2.2 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!4} -1.1 \\
\hline
Avg & \cellcolor{red!19} -4.8 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!12} -3.2 \\
\hline
\end{tabular}
}


==> images/minihack/metrics/forgetting_tables_10x.tex <==

\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllllllllllll|l|}
\hline
 & 0-RRand.. & 1-RDark & 2-RMons.. & 3-RTrap & 4-RUlti.. & 5-CorR2 & 6-CorR3 & 7-KeyRo.. & 8-KeyRo.. & 9-RivNa.. & 10-RivM.. & 11-RivL.. & 12-HnS & 13-HnS-.. & 14-CorB.. & Avg \\
\hline
0-RRand.. & \cellcolor{red!12} 3.1 & \cellcolor{red!4} 1.2 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 0.9 & \cellcolor{red!6} 1.6 & \cellcolor{red!5} 1.4 & \cellcolor{red!9} 2.5 & \cellcolor{red!13} 3.4 & \cellcolor{red!12} 3.2 & \cellcolor{red!12} 3.2 & \cellcolor{red!12} 3.1 & \cellcolor{red!14} 3.7 & \cellcolor{red!8} 2.2 & \cellcolor{red!5} 1.4 & \cellcolor{red!12} 3.1 & \cellcolor{red!9} 2.3 \\
1-RDark & \cellcolor{red!10} 2.7 & \cellcolor{red!7} 1.9 & \cellcolor{red!2} 0.6 & \cellcolor{red!8} 2.1 & \cellcolor{red!7} 1.9 & \cellcolor{red!7} 1.9 & \cellcolor{red!12} 3.1 & \cellcolor{red!12} 3.2 & \cellcolor{red!11} 2.9 & \cellcolor{red!12} 3.0 & \cellcolor{red!12} 3.2 & \cellcolor{red!14} 3.5 & \cellcolor{red!9} 2.3 & \cellcolor{red!5} 1.4 & \cellcolor{red!10} 2.7 & \cellcolor{red!9} 2.4 \\
2-RMons.. & \cellcolor{red!17} 4.5 & \cellcolor{red!16} 4.1 & \cellcolor{red!17} 4.5 & \cellcolor{red!9} 2.3 & \cellcolor{red!11} 2.9 & \cellcolor{red!10} 2.7 & \cellcolor{red!16} 4.2 & \cellcolor{red!21} 5.4 & \cellcolor{red!20} 5.2 & \cellcolor{red!21} 5.4 & \cellcolor{red!21} 5.3 & \cellcolor{red!24} 6.1 & \cellcolor{red!16} 4.2 & \cellcolor{red!10} 2.7 & \cellcolor{red!18} 4.6 & \cellcolor{red!17} 4.3 \\
3-RTrap & \cellcolor{red!22} 5.7 & \cellcolor{red!20} 5.0 & \cellcolor{red!20} 5.1 & \cellcolor{red!22} 5.5 & \cellcolor{red!14} 3.6 & \cellcolor{red!12} 3.2 & \cellcolor{red!17} 4.4 & \cellcolor{red!22} 5.6 & \cellcolor{red!21} 5.3 & \cellcolor{red!20} 5.1 & \cellcolor{red!18} 4.7 & \cellcolor{red!21} 5.4 & \cellcolor{red!17} 4.3 & \cellcolor{red!15} 3.9 & \cellcolor{red!21} 5.4 & \cellcolor{red!19} 4.8 \\
4-RUlti.. & \cellcolor{red!22} 5.6 & \cellcolor{red!19} 4.9 & \cellcolor{red!18} 4.6 & \cellcolor{red!23} 5.8 & \cellcolor{red!28} 7.0 & \cellcolor{red!15} 3.8 & \cellcolor{red!23} 6.0 & \cellcolor{red!22} 5.7 & \cellcolor{red!19} 4.9 & \cellcolor{red!19} 5.0 & \cellcolor{red!20} 5.2 & \cellcolor{red!22} 5.7 & \cellcolor{red!17} 4.5 & \cellcolor{red!14} 3.6 & \cellcolor{red!20} 5.1 & \cellcolor{red!20} 5.2 \\
5-CorR2 & \cellcolor{red!10} 2.6 & \cellcolor{red!11} 2.9 & \cellcolor{red!11} 3.0 & \cellcolor{red!10} 2.6 & \cellcolor{red!9} 2.3 & \cellcolor{red!9} 2.5 & \cellcolor{red!5} 1.3 & \cellcolor{red!9} 2.5 & \cellcolor{red!12} 3.1 & \cellcolor{red!13} 3.4 & \cellcolor{red!15} 3.8 & \cellcolor{red!15} 3.9 & \cellcolor{red!13} 3.3 & \cellcolor{red!9} 2.4 & \cellcolor{red!8} 2.1 & \cellcolor{red!11} 2.8 \\
6-CorR3 & \cellcolor{red!9} 2.4 & \cellcolor{red!10} 2.7 & \cellcolor{red!11} 2.9 & \cellcolor{red!10} 2.5 & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.2 & \cellcolor{red!8} 2.2 & \cellcolor{red!9} 2.3 & \cellcolor{red!11} 3.0 & \cellcolor{red!12} 3.2 & \cellcolor{red!14} 3.5 & \cellcolor{red!15} 3.8 & \cellcolor{red!11} 3.0 & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.0 & \cellcolor{red!10} 2.7 \\
7-KeyRo.. & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.1 & \cellcolor{red!8} 2.0 & \cellcolor{red!7} 2.0 & \cellcolor{red!8} 2.0 & \cellcolor{red!4} 1.1 & \cellcolor{red!3} 1.0 & \cellcolor{red!2} 0.7 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.2 & \cellcolor{red!2} 0.6 & \cellcolor{red!5} 1.4 & \cellcolor{red!7} 1.8 & \cellcolor{red!8} 2.0 & \cellcolor{red!8} 2.1 & \cellcolor{red!5} 1.4 \\
8-KeyRo.. & \cellcolor{red!9} 2.4 & \cellcolor{red!9} 2.4 & \cellcolor{red!9} 2.4 & \cellcolor{red!9} 2.3 & \cellcolor{red!8} 2.2 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.9 & \cellcolor{red!5} 1.3 & \cellcolor{red!3} 0.9 & \cellcolor{red!6} 1.7 & \cellcolor{red!8} 2.1 & \cellcolor{red!9} 2.3 & \cellcolor{red!9} 2.4 & \cellcolor{red!9} 2.4 & \cellcolor{red!8} 2.0 \\
9-RivNa.. & \cellcolor{green!2} -0.5 & \cellcolor{red!0} 0.1 & \cellcolor{red!1} 0.4 & \cellcolor{red!2} 0.5 & \cellcolor{red!5} 1.4 & \cellcolor{red!4} 1.1 & \cellcolor{red!5} 1.3 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.8 & \cellcolor{red!5} 1.3 & \cellcolor{green!11} -2.9 & \cellcolor{green!18} -4.7 & \cellcolor{green!12} -3.0 & \cellcolor{green!6} -1.6 & \cellcolor{green!3} -1.0 & \cellcolor{green!1} -0.3 \\
10-RivM.. & \cellcolor{red!4} 1.1 & \cellcolor{red!7} 1.8 & \cellcolor{red!7} 1.9 & \cellcolor{red!6} 1.7 & \cellcolor{red!9} 2.5 & \cellcolor{red!8} 2.0 & \cellcolor{red!7} 1.9 & \cellcolor{red!10} 2.6 & \cellcolor{red!12} 3.1 & \cellcolor{red!11} 2.9 & \cellcolor{red!5} 1.3 & \cellcolor{green!3} -1.0 & \cellcolor{green!2} -0.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!5} 1.5 \\
11-RivL.. & \cellcolor{red!9} 2.5 & \cellcolor{red!13} 3.3 & \cellcolor{red!13} 3.3 & \cellcolor{red!12} 3.1 & \cellcolor{red!15} 3.9 & \cellcolor{red!14} 3.6 & \cellcolor{red!14} 3.5 & \cellcolor{red!16} 4.2 & \cellcolor{red!18} 4.5 & \cellcolor{red!17} 4.4 & \cellcolor{red!11} 2.8 & \cellcolor{red!4} 1.0 & \cellcolor{red!3} 0.8 & \cellcolor{red!8} 2.0 & \cellcolor{red!7} 2.0 & \cellcolor{red!12} 3.0 \\
12-HnS & \cellcolor{red!12} 3.2 & \cellcolor{red!19} 4.8 & \cellcolor{red!21} 5.5 & \cellcolor{red!22} 5.7 & \cellcolor{red!25} 6.4 & \cellcolor{red!25} 6.4 & \cellcolor{red!25} 6.4 & \cellcolor{red!26} 6.7 & \cellcolor{red!27} 6.9 & \cellcolor{red!27} 6.9 & \cellcolor{red!26} 6.6 & \cellcolor{red!26} 6.6 & \cellcolor{red!17} 4.4 & \cellcolor{green!4} -1.0 & \cellcolor{red!5} 1.3 & \cellcolor{red!20} 5.1 \\
13-HnS-.. & \cellcolor{red!29} 7.3 & \cellcolor{red!34} 8.7 & \cellcolor{red!37} 9.4 & \cellcolor{red!38} 9.5 & \cellcolor{red!40} 10.2 & \cellcolor{red!40} 10.2 & \cellcolor{red!41} 10.3 & \cellcolor{red!42} 10.7 & \cellcolor{red!43} 10.8 & \cellcolor{red!42} 10.7 & \cellcolor{red!41} 10.4 & \cellcolor{red!41} 10.4 & \cellcolor{red!32} 8.1 & \cellcolor{red!23} 5.8 & \cellcolor{red!21} 5.3 & \cellcolor{red!36} 9.2 \\
14-CorB.. & \cellcolor{red!0} 0.0 & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.5 & \cellcolor{green!2} -0.7 & \cellcolor{green!4} -1.1 & \cellcolor{green!1} -0.3 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.0 & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.4 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.0 \\
\hline
Avg & \cellcolor{red!11} 3.0 & \cellcolor{red!12} 3.1 & \cellcolor{red!12} 3.1 & \cellcolor{red!12} 3.1 & \cellcolor{red!13} 3.4 & \cellcolor{red!11} 2.9 & \cellcolor{red!12} 3.2 & \cellcolor{red!15} 3.8 & \cellcolor{red!14} 3.7 & \cellcolor{red!14} 3.7 & \cellcolor{red!13} 3.3 & \cellcolor{red!12} 3.2 & \cellcolor{red!10} 2.5 & \cellcolor{red!7} 1.9 & \cellcolor{red!10} 2.5 & \cellcolor{red!11} 3.0 \\
\hline
\end{tabular}
}




\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllllllllllll|l|}
\hline
 & 0-RRand.. & 1-RDark & 2-RMons.. & 3-RTrap & 4-RUlti.. & 5-CorR2 & 6-CorR3 & 7-KeyRo.. & 8-KeyRo.. & 9-RivNa.. & 10-RivM.. & 11-RivL.. & 12-HnS & 13-HnS-.. & 14-CorB.. & Avg \\
\hline
0-RRand.. & \cellcolor{red!5} 1.5 & \cellcolor{red!2} 0.6 & \cellcolor{red!0} 0.2 & \cellcolor{green!0} -0.1 & \cellcolor{red!0} 0.1 & \cellcolor{green!0} -0.0 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.0 & \cellcolor{red!0} 0.1 & \cellcolor{green!0} -0.0 & \cellcolor{red!1} 0.3 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.5 & \cellcolor{red!3} 0.8 & \cellcolor{red!5} 1.3 & \cellcolor{red!1} 0.4 \\
1-RDark & \cellcolor{green!13} -3.4 & \cellcolor{green!15} -3.9 & \cellcolor{green!14} -3.6 & \cellcolor{green!16} -4.1 & \cellcolor{green!16} -4.0 & \cellcolor{green!17} -4.4 & \cellcolor{green!20} -5.0 & \cellcolor{green!21} -5.3 & \cellcolor{green!21} -5.5 & \cellcolor{green!21} -5.5 & \cellcolor{green!21} -5.3 & \cellcolor{green!20} -5.1 & \cellcolor{green!16} -4.0 & \cellcolor{green!10} -2.7 & \cellcolor{green!11} -3.0 & \cellcolor{green!17} -4.3 \\
2-RMons.. & \cellcolor{red!9} 2.5 & \cellcolor{red!10} 2.6 & \cellcolor{red!8} 2.2 & \cellcolor{red!2} 0.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.2 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.2 & \cellcolor{red!3} 0.9 & \cellcolor{red!6} 1.6 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 1.0 & \cellcolor{red!7} 1.9 & \cellcolor{red!4} 1.1 \\
3-RTrap & \cellcolor{red!10} 2.7 & \cellcolor{red!10} 2.7 & \cellcolor{red!11} 2.8 & \cellcolor{red!9} 2.5 & \cellcolor{red!5} 1.4 & \cellcolor{red!4} 1.1 & \cellcolor{red!2} 0.7 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.7 & \cellcolor{red!4} 1.0 & \cellcolor{red!6} 1.6 & \cellcolor{red!5} 1.5 & \cellcolor{red!7} 1.8 & \cellcolor{red!10} 2.7 & \cellcolor{red!6} 1.7 \\
4-RUlti.. & \cellcolor{red!2} 0.5 & \cellcolor{green!2} -0.6 & \cellcolor{green!4} -1.2 & \cellcolor{green!4} -1.0 & \cellcolor{green!4} -1.1 & \cellcolor{green!5} -1.3 & \cellcolor{green!7} -1.9 & \cellcolor{green!8} -2.2 & \cellcolor{green!8} -2.1 & \cellcolor{green!7} -2.0 & \cellcolor{green!8} -2.0 & \cellcolor{green!7} -2.0 & \cellcolor{green!4} -1.1 & \cellcolor{red!2} 0.6 & \cellcolor{red!4} 1.0 & \cellcolor{green!4} -1.1 \\
5-CorR2 & \cellcolor{red!6} 1.6 & \cellcolor{red!6} 1.6 & \cellcolor{red!6} 1.7 & \cellcolor{red!5} 1.4 & \cellcolor{red!5} 1.5 & \cellcolor{red!3} 0.8 & \cellcolor{red!0} 0.0 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.2 & \cellcolor{red!1} 0.3 & \cellcolor{red!3} 0.8 & \cellcolor{red!6} 1.5 & \cellcolor{red!3} 0.8 \\
6-CorR3 & \cellcolor{red!6} 1.5 & \cellcolor{red!5} 1.4 & \cellcolor{red!6} 1.5 & \cellcolor{red!5} 1.3 & \cellcolor{red!5} 1.4 & \cellcolor{red!2} 0.6 & \cellcolor{green!0} -0.1 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.3 & \cellcolor{green!0} -0.0 & \cellcolor{green!0} -0.2 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.2 & \cellcolor{red!3} 0.9 & \cellcolor{red!6} 1.6 & \cellcolor{red!2} 0.7 \\
7-KeyRo.. & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.0 & \cellcolor{red!1} 0.5 & \cellcolor{red!2} 0.5 & \cellcolor{red!2} 0.7 & \cellcolor{red!2} 0.6 & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.2 & \cellcolor{red!1} 0.4 & \cellcolor{red!3} 0.8 & \cellcolor{red!4} 1.1 & \cellcolor{red!3} 0.9 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.5 \\
8-KeyRo.. & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 1.0 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.0 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.0 & \cellcolor{red!3} 1.0 & \cellcolor{red!2} 0.7 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 0.9 & \cellcolor{red!3} 0.9 & \cellcolor{red!4} 1.0 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 1.0 \\
9-RivNa.. & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.0 & \cellcolor{green!0} -0.0 & \cellcolor{green!1} -0.5 & \cellcolor{green!2} -0.5 & \cellcolor{green!1} -0.4 & \cellcolor{green!1} -0.4 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.0 & \cellcolor{green!1} -0.5 & \cellcolor{green!5} -1.5 & \cellcolor{green!8} -2.1 & \cellcolor{green!5} -1.4 & \cellcolor{green!1} -0.3 & \cellcolor{red!1} 0.4 & \cellcolor{green!1} -0.5 \\
10-RivM.. & \cellcolor{red!7} 1.9 & \cellcolor{red!6} 1.7 & \cellcolor{red!4} 1.2 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 0.9 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 0.9 & \cellcolor{red!4} 1.0 & \cellcolor{red!4} 1.2 & \cellcolor{red!5} 1.4 & \cellcolor{red!5} 1.3 & \cellcolor{red!1} 0.4 & \cellcolor{red!2} 0.7 & \cellcolor{red!5} 1.5 & \cellcolor{red!8} 2.0 & \cellcolor{red!4} 1.2 \\
11-RivL.. & \cellcolor{red!6} 1.7 & \cellcolor{red!5} 1.5 & \cellcolor{red!3} 1.0 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 1.0 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 1.0 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.2 & \cellcolor{red!4} 1.1 & \cellcolor{red!2} 0.6 & \cellcolor{red!2} 0.6 & \cellcolor{red!5} 1.4 & \cellcolor{red!7} 1.9 & \cellcolor{red!4} 1.1 \\
12-HnS & \cellcolor{red!4} 1.2 & \cellcolor{red!6} 1.6 & \cellcolor{red!7} 1.9 & \cellcolor{red!8} 2.2 & \cellcolor{red!9} 2.4 & \cellcolor{red!10} 2.7 & \cellcolor{red!11} 2.9 & \cellcolor{red!11} 2.9 & \cellcolor{red!9} 2.5 & \cellcolor{red!9} 2.3 & \cellcolor{red!9} 2.3 & \cellcolor{red!10} 2.5 & \cellcolor{green!6} -1.7 & \cellcolor{green!19} -4.8 & \cellcolor{green!5} -1.5 & \cellcolor{red!5} 1.3 \\
13-HnS-.. & \cellcolor{red!23} 5.9 & \cellcolor{red!24} 6.1 & \cellcolor{red!26} 6.7 & \cellcolor{red!26} 6.7 & \cellcolor{red!26} 6.7 & \cellcolor{red!27} 6.9 & \cellcolor{red!26} 6.7 & \cellcolor{red!27} 6.8 & \cellcolor{red!27} 6.8 & \cellcolor{red!27} 6.9 & \cellcolor{red!28} 7.1 & \cellcolor{red!28} 7.1 & \cellcolor{red!11} 2.8 & \cellcolor{red!0} 0.0 & \cellcolor{red!12} 3.2 & \cellcolor{red!23} 5.8 \\
14-CorB.. & \cellcolor{green!2} -0.7 & \cellcolor{green!1} -0.3 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.2 & \cellcolor{green!1} -0.3 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.0 & \cellcolor{green!1} -0.3 & \cellcolor{green!1} -0.4 & \cellcolor{green!0} -0.2 & \cellcolor{red!1} 0.3 & \cellcolor{red!2} 0.7 & \cellcolor{red!0} 0.2 & \cellcolor{green!0} -0.1 \\
\hline
Avg & \cellcolor{red!4} 1.2 & \cellcolor{red!4} 1.1 & \cellcolor{red!4} 1.1 & \cellcolor{red!3} 0.8 & \cellcolor{red!3} 0.8 & \cellcolor{red!2} 0.6 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.5 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.4 & \cellcolor{red!2} 0.5 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.2 & \cellcolor{red!3} 1.0 & \cellcolor{red!1} 0.4 \\
\hline
\end{tabular}
}



==> images/minihack/metrics/forgetting_tables_10x_old.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|llllllllllllllllllllllllllllll|}
\hline
{} & {0-Room-Random (C0)} & {1-Room-Dark (C0)} & {2-Room-Monster (C0)} & {3-Room-Trap (C0)} & {4-Room-Ultimate (C0)} & {5-Corridor-R2 (C0)} & {6-Corridor-R3 (C0)} & {7-KeyRoom (C0)} & {8-KeyRoom-Dark (C0)} & {9-River-Narrow (C0)} & {10-River-Monster (C0)} & {11-River-Lava (C0)} & {12-HideNSeek (C0)} & {13-HideNSeek-Lava (C0)} & {14-CorridorBattle (C0)} & {0-Room-Random (C1)} & {1-Room-Dark (C1)} & {2-Room-Monster (C1)} & {3-Room-Trap (C1)} & {4-Room-Ultimate (C1)} & {5-Corridor-R2 (C1)} & {6-Corridor-R3 (C1)} & {7-KeyRoom (C1)} & {8-KeyRoom-Dark (C1)} & {9-River-Narrow (C1)} & {10-River-Monster (C1)} & {11-River-Lava (C1)} & {12-HideNSeek (C1)} & {13-HideNSeek-Lava (C1)} & {14-CorridorBattle (C1)} \\
0-Room-Random & \cellcolor{white!20} -- & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -0.8 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -1.3 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.8 & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -1.5 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.4 & \cellcolor{white!20} -0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 0.7 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 1.0 \\
1-Room-Dark & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 0.9 & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.5 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.2 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -1.0 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{green!20} -0.4 & \cellcolor{white!20} -0.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 1.1 \\
2-Room-Monster & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -0.1 & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.8 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.4 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 2.8 \\
3-Room-Trap & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.1 & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 2.7 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 2.4 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 2.9 \\
4-Room-Ultimate & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 2.4 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 2.9 \\
5-Corridor-R2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -0.0 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 2.7 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 0.4 \\
6-Corridor-R3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 2.7 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 0.7 \\
7-KeyRoom & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.8 & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.1 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -0.0 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 \\
8-KeyRoom-Dark & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.1 \\
9-River-Narrow & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -1.8 & \cellcolor{green!20} -2.8 & \cellcolor{green!20} -2.1 & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.3 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.3 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -1.3 & \cellcolor{green!20} -1.3 & \cellcolor{green!20} -1.1 & \cellcolor{green!20} -0.9 \\
10-River-Monster & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.6 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 0.8 & \cellcolor{white!20} -0.1 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 \\
11-River-Lava & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.9 \\
12-HideNSeek & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -2.1 & \cellcolor{green!20} -0.3 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 3.2 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 1.9 & \cellcolor{white!20} -0.1 & \cellcolor{red!20} 1.0 \\
13-HideNSeek-Lava & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 4.8 & \cellcolor{red!20} 5.4 & \cellcolor{red!20} 5.5 & \cellcolor{red!20} 6.0 & \cellcolor{red!20} 5.9 & \cellcolor{red!20} 6.0 & \cellcolor{red!20} 6.4 & \cellcolor{red!20} 6.4 & \cellcolor{red!20} 6.3 & \cellcolor{red!20} 6.1 & \cellcolor{red!20} 6.2 & \cellcolor{red!20} 4.2 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 3.3 \\
14-CorridorBattle & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.1 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llllllllllllllllllllllllllllll|}
\hline
{} & {0-Room-Random (C0)} & {1-Room-Dark (C0)} & {2-Room-Monster (C0)} & {3-Room-Trap (C0)} & {4-Room-Ultimate (C0)} & {5-Corridor-R2 (C0)} & {6-Corridor-R3 (C0)} & {7-KeyRoom (C0)} & {8-KeyRoom-Dark (C0)} & {9-River-Narrow (C0)} & {10-River-Monster (C0)} & {11-River-Lava (C0)} & {12-HideNSeek (C0)} & {13-HideNSeek-Lava (C0)} & {14-CorridorBattle (C0)} & {0-Room-Random (C1)} & {1-Room-Dark (C1)} & {2-Room-Monster (C1)} & {3-Room-Trap (C1)} & {4-Room-Ultimate (C1)} & {5-Corridor-R2 (C1)} & {6-Corridor-R3 (C1)} & {7-KeyRoom (C1)} & {8-KeyRoom-Dark (C1)} & {9-River-Narrow (C1)} & {10-River-Monster (C1)} & {11-River-Lava (C1)} & {12-HideNSeek (C1)} & {13-HideNSeek-Lava (C1)} & {14-CorridorBattle (C1)} \\
0-Room-Random & \cellcolor{white!20} -- & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -1.3 & \cellcolor{green!20} -1.4 & \cellcolor{green!20} -1.6 & \cellcolor{green!20} -1.5 & \cellcolor{green!20} -1.6 & \cellcolor{green!20} -1.5 & \cellcolor{green!20} -1.6 & \cellcolor{white!20} -0.0 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.2 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 2.6 \\
1-Room-Dark & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -2.5 & \cellcolor{green!20} -3.2 & \cellcolor{green!20} -2.9 & \cellcolor{green!20} -3.1 & \cellcolor{green!20} -3.3 & \cellcolor{green!20} -2.8 & \cellcolor{green!20} -3.0 & \cellcolor{green!20} -3.5 & \cellcolor{green!20} -3.1 & \cellcolor{green!20} -3.0 & \cellcolor{green!20} -2.8 & \cellcolor{green!20} -2.9 & \cellcolor{green!20} -3.9 & \cellcolor{green!20} -4.4 & \cellcolor{green!20} -3.8 & \cellcolor{green!20} -4.1 & \cellcolor{green!20} -4.9 & \cellcolor{green!20} -4.8 & \cellcolor{green!20} -4.9 & \cellcolor{green!20} -5.1 & \cellcolor{green!20} -5.5 & \cellcolor{green!20} -5.7 & \cellcolor{green!20} -5.4 & \cellcolor{green!20} -4.8 & \cellcolor{green!20} -4.3 & \cellcolor{green!20} -4.1 & \cellcolor{green!20} -3.8 & \cellcolor{green!20} -4.4 \\
2-Room-Monster & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -1.1 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -1.3 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.3 & \cellcolor{red!20} 3.2 & \cellcolor{red!20} 4.4 & \cellcolor{red!20} 4.6 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.2 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.8 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 2.6 & \cellcolor{red!20} 2.7 & \cellcolor{red!20} 3.2 \\
3-Room-Trap & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -0.0 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.6 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.0 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 4.1 & \cellcolor{red!20} 4.3 & \cellcolor{red!20} 4.2 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 4.4 & \cellcolor{red!20} 4.3 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 3.9 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.8 \\
4-Room-Ultimate & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -1.1 & \cellcolor{green!20} -0.9 & \cellcolor{red!20} 0.2 & \cellcolor{white!20} 0.0 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -1.7 & \cellcolor{green!20} -1.6 & \cellcolor{green!20} -1.7 & \cellcolor{green!20} -1.8 & \cellcolor{green!20} -1.9 & \cellcolor{green!20} -2.3 & \cellcolor{green!20} -2.4 & \cellcolor{green!20} -2.2 & \cellcolor{green!20} -2.0 & \cellcolor{green!20} -1.8 & \cellcolor{green!20} -1.6 & \cellcolor{green!20} -0.5 & \cellcolor{white!20} 0.0 \\
5-Corridor-R2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 0.2 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -1.5 & \cellcolor{green!20} -1.6 & \cellcolor{green!20} -0.8 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 2.1 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 0.8 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.6 & \cellcolor{white!20} -0.1 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.7 \\
6-Corridor-R3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.7 & \cellcolor{green!20} -0.1 & \cellcolor{green!20} -1.0 & \cellcolor{green!20} -1.9 & \cellcolor{green!20} -1.9 & \cellcolor{green!20} -1.1 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 0.4 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.8 & \cellcolor{green!20} -0.5 & \cellcolor{white!20} -0.0 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 2.4 \\
7-KeyRoom & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.3 & \cellcolor{white!20} -0.1 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.1 & \cellcolor{green!20} -0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} -0.0 & \cellcolor{green!20} -0.1 & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.4 \\
8-KeyRoom-Dark & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 \\
9-River-Narrow & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.3 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.3 & \cellcolor{white!20} 0.1 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{white!20} -0.0 & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.5 \\
10-River-Monster & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.4 \\
11-River-Lava & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.9 \\
12-HideNSeek & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -2.1 & \cellcolor{green!20} -0.3 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 1.6 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 1.7 & \cellcolor{red!20} 0.1 & \cellcolor{green!20} -1.3 & \cellcolor{red!20} 0.3 \\
13-HideNSeek-Lava & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 3.1 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.4 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.3 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.5 & \cellcolor{red!20} 3.6 & \cellcolor{red!20} 3.7 & \cellcolor{red!20} 2.2 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 2.0 \\
14-CorridorBattle & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.3 & \cellcolor{white!20} -0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} -0.1 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} -0.1 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} -0.1 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 \\
\hline
\end{tabular}
}

==> images/minihack/metrics/transfer_tables_10x.tex <==

\subfloat[IMPALA]{ 
 \begin{tabular}{|l|llllllllllllllH|l|}
\hline
{} & {0-RRand..} & {1-RDark} & {2-RMons..} & {3-RTrap} & {4-RUlti..} & {5-CorR2} & {6-CorR3} & {7-KeyRo..} & {8-KeyRo..} & {9-RivNa..} & {10-RivM..} & {11-RivL..} & {12-HnS} & {13-HnS-..} & {14-CorB..} & {Avg} \\
\hline
0-RRand.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-RDark & \cellcolor{green!14} 3.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.7 \\
2-RMons.. & \cellcolor{green!37} 9.4 & \cellcolor{green!39} 10.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!38} 9.7 \\
3-RTrap & \cellcolor{green!31} 7.9 & \cellcolor{green!39} 9.8 & \cellcolor{green!46} 11.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!39} 9.8 \\
4-RUlti.. & \cellcolor{green!26} 6.6 & \cellcolor{green!41} 10.5 & \cellcolor{green!43} 11.0 & \cellcolor{green!28} 7.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!35} 8.8 \\
5-CorR2 & \cellcolor{green!12} 3.1 & \cellcolor{green!11} 3.0 & \cellcolor{green!14} 3.6 & \cellcolor{green!16} 4.2 & \cellcolor{green!13} 3.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!13} 3.5 \\
6-CorR3 & \cellcolor{green!13} 3.5 & \cellcolor{green!12} 3.1 & \cellcolor{green!14} 3.6 & \cellcolor{green!16} 4.2 & \cellcolor{green!13} 3.4 & \cellcolor{green!18} 4.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.7 \\
7-KeyRo.. & \cellcolor{green!1} 0.4 & \cellcolor{green!2} 0.5 & \cellcolor{green!7} 2.0 & \cellcolor{green!12} 3.1 & \cellcolor{green!9} 2.3 & \cellcolor{green!20} 5.2 & \cellcolor{green!21} 5.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!10} 2.7 \\
8-KeyRo.. & \cellcolor{green!21} 5.3 & \cellcolor{green!12} 3.0 & \cellcolor{green!12} 3.0 & \cellcolor{green!20} 5.2 & \cellcolor{green!11} 2.9 & \cellcolor{green!15} 4.0 & \cellcolor{green!16} 4.2 & \cellcolor{green!7} 2.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.7 \\
9-RivNa.. & \cellcolor{green!26} 6.6 & \cellcolor{green!26} 6.7 & \cellcolor{green!26} 6.7 & \cellcolor{green!27} 7.0 & \cellcolor{green!25} 6.4 & \cellcolor{green!24} 6.0 & \cellcolor{green!16} 4.1 & \cellcolor{green!13} 3.5 & \cellcolor{green!14} 3.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!22} 5.6 \\
10-RivM.. & \cellcolor{green!31} 8.0 & \cellcolor{green!30} 7.6 & \cellcolor{green!29} 7.5 & \cellcolor{green!32} 8.1 & \cellcolor{green!30} 7.5 & \cellcolor{green!27} 6.9 & \cellcolor{green!18} 4.7 & \cellcolor{green!13} 3.3 & \cellcolor{green!11} 2.8 & \cellcolor{green!14} 3.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!23} 6.0 \\
11-RivL.. & \cellcolor{green!32} 8.0 & \cellcolor{green!30} 7.7 & \cellcolor{green!30} 7.6 & \cellcolor{green!31} 8.0 & \cellcolor{green!30} 7.5 & \cellcolor{green!27} 6.8 & \cellcolor{green!17} 4.5 & \cellcolor{green!12} 3.2 & \cellcolor{green!11} 2.9 & \cellcolor{green!15} 3.8 & \cellcolor{green!26} 6.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!24} 6.1 \\
12-HnS & \cellcolor{green!16} 4.0 & \cellcolor{green!8} 2.1 & \cellcolor{green!3} 0.9 & \cellcolor{green!9} 2.4 & \cellcolor{green!7} 1.8 & \cellcolor{green!4} 1.0 & \cellcolor{green!0} 0.1 & \cellcolor{green!2} 0.6 & \cellcolor{green!8} 2.2 & \cellcolor{green!6} 1.7 & \cellcolor{green!4} 1.1 & \cellcolor{green!5} 1.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!6} 1.6 \\
13-HnS-.. & \cellcolor{green!22} 5.6 & \cellcolor{green!15} 3.8 & \cellcolor{green!11} 2.8 & \cellcolor{green!17} 4.3 & \cellcolor{green!14} 3.5 & \cellcolor{green!9} 2.3 & \cellcolor{green!6} 1.6 & \cellcolor{green!10} 2.5 & \cellcolor{green!16} 4.1 & \cellcolor{green!14} 3.7 & \cellcolor{green!12} 3.1 & \cellcolor{green!10} 2.7 & \cellcolor{green!38} 9.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!15} 3.8 \\
14-CorB.. & \cellcolor{green!19} 4.9 & \cellcolor{green!11} 2.8 & \cellcolor{green!8} 2.1 & \cellcolor{green!15} 3.9 & \cellcolor{green!8} 2.2 & \cellcolor{green!10} 2.7 & \cellcolor{green!12} 3.1 & \cellcolor{green!10} 2.7 & \cellcolor{green!13} 3.4 & \cellcolor{green!11} 2.8 & \cellcolor{green!7} 1.8 & \cellcolor{green!2} 0.6 & \cellcolor{green!2} 0.5 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!9} 2.4 \\
\hline
Avg & \cellcolor{green!22} 5.5 & \cellcolor{green!21} 5.4 & \cellcolor{green!20} 5.2 & \cellcolor{green!20} 5.2 & \cellcolor{green!16} 4.1 & \cellcolor{green!17} 4.4 & \cellcolor{green!13} 3.5 & \cellcolor{green!10} 2.5 & \cellcolor{green!12} 3.2 & \cellcolor{green!12} 3.1 & \cellcolor{green!12} 3.2 & \cellcolor{green!6} 1.5 & \cellcolor{green!20} 5.1 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!17} 4.3 \\
\hline
\end{tabular}
}




\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llllllllllllllH|l|}
\hline
{} & {0-RRand..} & {1-RDark} & {2-RMons..} & {3-RTrap} & {4-RUlti..} & {5-CorR2} & {6-CorR3} & {7-KeyRo..} & {8-KeyRo..} & {9-RivNa..} & {10-RivM..} & {11-RivL..} & {12-HnS} & {13-HnS-..} & {14-CorB..} & {Avg} \\
\hline
0-RRand.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-RDark & \cellcolor{green!11} 3.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!11} 3.0 \\
2-RMons.. & \cellcolor{green!33} 8.3 & \cellcolor{green!34} 8.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!34} 8.5 \\
3-RTrap & \cellcolor{green!36} 9.0 & \cellcolor{green!39} 9.9 & \cellcolor{green!43} 10.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!39} 9.9 \\
4-RUlti.. & \cellcolor{green!12} 3.0 & \cellcolor{green!20} 5.1 & \cellcolor{green!32} 8.2 & \cellcolor{green!35} 8.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!25} 6.3 \\
5-CorR2 & \cellcolor{green!10} 2.6 & \cellcolor{green!10} 2.7 & \cellcolor{green!15} 4.0 & \cellcolor{green!17} 4.4 & \cellcolor{green!13} 3.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!13} 3.4 \\
6-CorR3 & \cellcolor{green!10} 2.7 & \cellcolor{green!11} 2.8 & \cellcolor{green!16} 4.1 & \cellcolor{green!17} 4.4 & \cellcolor{green!14} 3.5 & \cellcolor{green!18} 4.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.7 \\
7-KeyRo.. & \cellcolor{green!10} 2.6 & \cellcolor{green!10} 2.7 & \cellcolor{green!18} 4.6 & \cellcolor{green!19} 4.8 & \cellcolor{green!12} 3.1 & \cellcolor{green!19} 5.0 & \cellcolor{green!21} 5.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!16} 4.0 \\
8-KeyRo.. & \cellcolor{green!17} 4.4 & \cellcolor{green!10} 2.7 & \cellcolor{green!2} 0.6 & \cellcolor{green!0} 0.1 & \cellcolor{green!0} 0.0 & \cellcolor{green!0} 0.2 & \cellcolor{green!2} 0.5 & \cellcolor{green!5} 1.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!4} 1.2 \\
9-RivNa.. & \cellcolor{green!15} 3.8 & \cellcolor{green!16} 4.1 & \cellcolor{green!15} 4.0 & \cellcolor{green!14} 3.7 & \cellcolor{green!14} 3.7 & \cellcolor{green!14} 3.7 & \cellcolor{green!13} 3.4 & \cellcolor{green!12} 3.1 & \cellcolor{green!11} 2.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.6 \\
10-RivM.. & \cellcolor{green!23} 5.8 & \cellcolor{green!23} 5.9 & \cellcolor{green!22} 5.7 & \cellcolor{green!22} 5.5 & \cellcolor{green!21} 5.5 & \cellcolor{green!20} 5.2 & \cellcolor{green!17} 4.5 & \cellcolor{green!15} 3.9 & \cellcolor{green!15} 3.8 & \cellcolor{green!15} 3.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!19} 5.0 \\
11-RivL.. & \cellcolor{green!19} 4.9 & \cellcolor{green!20} 5.2 & \cellcolor{green!20} 5.1 & \cellcolor{green!18} 4.7 & \cellcolor{green!18} 4.6 & \cellcolor{green!17} 4.5 & \cellcolor{green!15} 3.8 & \cellcolor{green!12} 3.2 & \cellcolor{green!11} 2.9 & \cellcolor{green!10} 2.7 & \cellcolor{green!10} 2.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!16} 4.0 \\
12-HnS & \cellcolor{green!14} 3.6 & \cellcolor{green!12} 3.1 & \cellcolor{green!9} 2.3 & \cellcolor{green!6} 1.7 & \cellcolor{green!7} 1.9 & \cellcolor{green!7} 1.8 & \cellcolor{green!3} 0.9 & \cellcolor{green!2} 0.7 & \cellcolor{green!4} 1.2 & \cellcolor{green!6} 1.7 & \cellcolor{green!8} 2.1 & \cellcolor{green!9} 2.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.9 \\
13-HnS-.. & \cellcolor{green!10} 2.6 & \cellcolor{green!8} 2.1 & \cellcolor{green!5} 1.3 & \cellcolor{green!4} 1.1 & \cellcolor{green!4} 1.2 & \cellcolor{green!2} 0.7 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.2 & \cellcolor{green!2} 0.5 & \cellcolor{green!2} 0.7 & \cellcolor{green!2} 0.6 & \cellcolor{green!3} 1.0 & \cellcolor{green!25} 6.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!5} 1.4 \\
14-CorB.. & \cellcolor{green!7} 1.9 & \cellcolor{green!4} 1.1 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{green!2} 0.7 & \cellcolor{green!5} 1.4 & \cellcolor{green!4} 1.0 & \cellcolor{green!2} 0.5 & \cellcolor{green!1} 0.3 & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.1 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!2} 0.5 \\
\hline
Avg & \cellcolor{green!16} 4.2 & \cellcolor{green!17} 4.3 & \cellcolor{green!16} 4.2 & \cellcolor{green!14} 3.6 & \cellcolor{green!10} 2.7 & \cellcolor{green!11} 2.9 & \cellcolor{green!9} 2.4 & \cellcolor{green!7} 1.9 & \cellcolor{green!8} 2.1 & \cellcolor{green!7} 1.9 & \cellcolor{green!5} 1.4 & \cellcolor{green!4} 1.1 & \cellcolor{green!12} 3.2 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!12} 3.1 \\
\hline
\end{tabular}
}




==> images/minihack/metrics/transfer_tables_10x_isolated.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|llllllllllllllH|l|}
\hline
 & 0-RRand.. & 1-RDark & 2-RMons.. & 3-RTrap & 4-RUlti.. & 5-CorR2 & 6-CorR3 & 7-KeyRo.. & 8-KeyRo.. & 9-RivNa.. & 10-RivM.. & 11-RivL.. & 12-HnS & 13-HnS-.. & 14-CorB.. & Avg \\
\hline
0-RRand.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-RDark & \cellcolor{green!16} 4.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!16} 4.0 \\
2-RMons.. & \cellcolor{green!34} 8.6 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!17} 4.4 \\
3-RTrap & \cellcolor{green!29} 7.5 & \cellcolor{green!3} 0.9 & \cellcolor{green!4} 1.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!12} 3.2 \\
4-RUlti.. & \cellcolor{green!23} 5.8 & \cellcolor{green!11} 3.0 & \cellcolor{green!4} 1.1 & \cellcolor{red!8} -2.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.9 \\
5-CorR2 & \cellcolor{green!12} 3.2 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.4 & \cellcolor{green!0} 0.2 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!2} 0.7 \\
6-CorR3 & \cellcolor{green!12} 3.2 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.5 & \cellcolor{green!0} 0.2 & \cellcolor{red!2} -0.5 & \cellcolor{green!5} 1.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
7-KeyRo.. & \cellcolor{green!4} 1.1 & \cellcolor{green!1} 0.3 & \cellcolor{green!5} 1.3 & \cellcolor{green!3} 0.9 & \cellcolor{red!0} -0.2 & \cellcolor{green!9} 2.3 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
8-KeyRo.. & \cellcolor{green!12} 3.1 & \cellcolor{red!3} -1.0 & \cellcolor{green!1} 0.5 & \cellcolor{green!5} 1.5 & \cellcolor{red!5} -1.3 & \cellcolor{green!4} 1.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!8} -2.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
9-RivNa.. & \cellcolor{green!25} 6.4 & \cellcolor{red!0} -0.1 & \cellcolor{green!0} 0.1 & \cellcolor{green!1} 0.4 & \cellcolor{red!1} -0.5 & \cellcolor{red!1} -0.4 & \cellcolor{red!7} -2.0 & \cellcolor{red!2} -0.7 & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
10-RivM.. & \cellcolor{green!28} 7.2 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -0.0 & \cellcolor{green!2} 0.5 & \cellcolor{red!3} -0.8 & \cellcolor{red!2} -0.6 & \cellcolor{red!7} -1.8 & \cellcolor{red!4} -1.0 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.3 \\
11-RivL.. & \cellcolor{green!28} 7.1 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -0.0 & \cellcolor{green!1} 0.5 & \cellcolor{red!3} -0.8 & \cellcolor{red!3} -0.8 & \cellcolor{red!7} -1.9 & \cellcolor{red!3} -1.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.1 & \cellcolor{green!6} 1.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
12-HnS & \cellcolor{green!18} 4.7 & \cellcolor{red!6} -1.5 & \cellcolor{red!3} -0.8 & \cellcolor{green!4} 1.2 & \cellcolor{red!3} -0.8 & \cellcolor{red!2} -0.7 & \cellcolor{red!2} -0.6 & \cellcolor{red!0} -0.0 & \cellcolor{green!2} 0.7 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
13-HnS-.. & \cellcolor{green!21} 5.4 & \cellcolor{red!5} -1.5 & \cellcolor{red!2} -0.7 & \cellcolor{green!4} 1.2 & \cellcolor{red!3} -0.9 & \cellcolor{red!3} -0.8 & \cellcolor{red!1} -0.5 & \cellcolor{green!0} 0.2 & \cellcolor{green!2} 0.7 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!2} -0.5 & \cellcolor{green!20} 5.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!2} 0.6 \\
14-CorB.. & \cellcolor{green!17} 4.4 & \cellcolor{red!5} -1.5 & \cellcolor{red!0} -0.0 & \cellcolor{green!5} 1.4 & \cellcolor{red!5} -1.5 & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.5 & \cellcolor{red!3} -0.9 & \cellcolor{red!3} -0.9 & \cellcolor{red!2} -0.7 & \cellcolor{green!0} 0.1 & \cellcolor{red!1} -0.5 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
\hline
Avg & \cellcolor{green!20} 5.1 & \cellcolor{red!0} -0.2 & \cellcolor{green!1} 0.3 & \cellcolor{green!2} 0.5 & \cellcolor{red!3} -0.8 & \cellcolor{green!0} 0.2 & \cellcolor{red!3} -0.9 & \cellcolor{red!2} -0.7 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.1 & \cellcolor{red!1} -0.5 & \cellcolor{green!10} 2.7 & \cellcolor{red!1} -0.5 & \cellcolor{red!0} -- & \cellcolor{green!2} 0.6 \\
\hline
\end{tabular}
}




\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llllllllllllllH|l|}
\hline
 & 0-RRand.. & 1-RDark & 2-RMons.. & 3-RTrap & 4-RUlti.. & 5-CorR2 & 6-CorR3 & 7-KeyRo.. & 8-KeyRo.. & 9-RivNa.. & 10-RivM.. & 11-RivL.. & 12-HnS & 13-HnS-.. & 14-CorB.. & Avg \\
\hline
0-RRand.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-RDark & \cellcolor{green!9} 2.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!9} 2.5 \\
2-RMons.. & \cellcolor{green!28} 7.1 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!14} 3.6 \\
3-RTrap & \cellcolor{green!28} 7.0 & \cellcolor{green!2} 0.7 & \cellcolor{green!3} 0.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!11} 2.9 \\
4-RUlti.. & \cellcolor{green!8} 2.1 & \cellcolor{green!9} 2.3 & \cellcolor{green!10} 2.7 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.8 \\
5-CorR2 & \cellcolor{green!6} 1.5 & \cellcolor{green!0} 0.2 & \cellcolor{green!3} 0.8 & \cellcolor{green!0} 0.1 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
6-CorR3 & \cellcolor{green!6} 1.6 & \cellcolor{green!0} 0.1 & \cellcolor{green!3} 0.9 & \cellcolor{green!0} 0.2 & \cellcolor{red!2} -0.6 & \cellcolor{green!3} 0.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!2} 0.5 \\
7-KeyRo.. & \cellcolor{green!5} 1.3 & \cellcolor{green!0} 0.0 & \cellcolor{green!3} 1.0 & \cellcolor{green!0} 0.1 & \cellcolor{red!3} -0.9 & \cellcolor{green!5} 1.5 & \cellcolor{green!2} 0.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!2} 0.5 \\
8-KeyRo.. & \cellcolor{green!8} 2.2 & \cellcolor{red!3} -0.9 & \cellcolor{red!4} -1.0 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.0 & \cellcolor{green!1} 0.3 & \cellcolor{green!1} 0.3 & \cellcolor{green!2} 0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
9-RivNa.. & \cellcolor{green!9} 2.5 & \cellcolor{green!1} 0.5 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.1 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.3 \\
10-RivM.. & \cellcolor{green!12} 3.0 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!2} -0.5 & \cellcolor{red!2} -0.7 & \cellcolor{green!0} 0.1 & \cellcolor{green!2} 0.5 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
11-RivL.. & \cellcolor{green!11} 2.8 & \cellcolor{green!1} 0.3 & \cellcolor{green!0} 0.0 & \cellcolor{red!1} -0.4 & \cellcolor{red!1} -0.3 & \cellcolor{red!1} -0.3 & \cellcolor{red!1} -0.5 & \cellcolor{red!0} -0.0 & \cellcolor{green!1} 0.4 & \cellcolor{red!1} -0.3 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
12-HnS & \cellcolor{green!10} 2.6 & \cellcolor{red!2} -0.7 & \cellcolor{red!3} -0.8 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -0.0 & \cellcolor{green!2} 0.6 & \cellcolor{green!1} 0.4 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
13-HnS-.. & \cellcolor{green!9} 2.3 & \cellcolor{red!2} -0.6 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.0 & \cellcolor{green!2} 0.5 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!15} 3.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.4 \\
14-CorB.. & \cellcolor{green!3} 0.8 & \cellcolor{red!1} -0.4 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -0.1 & \cellcolor{green!0} 0.0 & \cellcolor{green!0} 0.1 & \cellcolor{green!3} 0.8 & \cellcolor{green!5} 1.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!3} -0.9 & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -0.0 & \cellcolor{red!1} -0.3 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
Avg & \cellcolor{green!11} 2.8 & \cellcolor{green!0} 0.1 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!1} -0.3 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.3 & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.0 & \cellcolor{green!7} 1.8 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -- & \cellcolor{green!1} 0.5 \\
\hline
\end{tabular}
}



==> images/minihack/metrics/transfer_tables_10x_old.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllllllllllll|}
\hline
{} & {0-Room-Random (C0)} & {1-Room-Dark (C0)} & {2-Room-Monster (C0)} & {3-Room-Trap (C0)} & {4-Room-Ultimate (C0)} & {5-Corridor-R2 (C0)} & {6-Corridor-R3 (C0)} & {7-KeyRoom (C0)} & {8-KeyRoom-Dark (C0)} & {9-River-Narrow (C0)} & {10-River-Monster (C0)} & {11-River-Lava (C0)} & {12-HideNSeek (C0)} & {13-HideNSeek-Lava (C0)} & {14-CorridorBattle (C0)} \\
0-Room-Random & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Room-Dark & \cellcolor{green!20} 1.8 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Room-Monster & \cellcolor{green!20} 5.1 & \cellcolor{green!20} 5.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Room-Trap & \cellcolor{green!20} 5.0 & \cellcolor{green!20} 6.2 & \cellcolor{green!20} 7.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Room-Ultimate & \cellcolor{green!20} 3.2 & \cellcolor{green!20} 5.1 & \cellcolor{green!20} 5.4 & \cellcolor{green!20} 3.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Corridor-R2 & \cellcolor{green!20} 3.1 & \cellcolor{green!20} 3.0 & \cellcolor{green!20} 3.6 & \cellcolor{green!20} 4.2 & \cellcolor{green!20} 3.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
6-Corridor-R3 & \cellcolor{green!20} 3.5 & \cellcolor{green!20} 3.1 & \cellcolor{green!20} 3.6 & \cellcolor{green!20} 4.2 & \cellcolor{green!20} 3.4 & \cellcolor{green!20} 4.6 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
7-KeyRoom & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 0.9 & \cellcolor{green!20} 2.1 & \cellcolor{green!20} 2.2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
8-KeyRoom-Dark & \cellcolor{green!20} 2.1 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 2.1 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.7 & \cellcolor{green!20} 0.8 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
9-River-Narrow & \cellcolor{green!20} 2.3 & \cellcolor{green!20} 2.3 & \cellcolor{green!20} 2.3 & \cellcolor{green!20} 2.4 & \cellcolor{green!20} 2.2 & \cellcolor{green!20} 2.1 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 1.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
10-River-Monster & \cellcolor{green!20} 2.8 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.8 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.4 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 1.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
11-River-Lava & \cellcolor{green!20} 2.8 & \cellcolor{green!20} 2.7 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.8 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.4 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 2.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
12-HideNSeek & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 0.9 & \cellcolor{green!20} 0.4 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 0.5 & \cellcolor{white!20} 0.1 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.6 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
13-HideNSeek-Lava & \cellcolor{green!20} 2.5 & \cellcolor{green!20} 1.7 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 1.9 & \cellcolor{green!20} 1.5 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 4.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
14-CorridorBattle & \cellcolor{green!20} 1.7 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 0.9 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.6 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.2 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllllllllllll|}
\hline
{} & {0-Room-Random (C0)} & {1-Room-Dark (C0)} & {2-Room-Monster (C0)} & {3-Room-Trap (C0)} & {4-Room-Ultimate (C0)} & {5-Corridor-R2 (C0)} & {6-Corridor-R3 (C0)} & {7-KeyRoom (C0)} & {8-KeyRoom-Dark (C0)} & {9-River-Narrow (C0)} & {10-River-Monster (C0)} & {11-River-Lava (C0)} & {12-HideNSeek (C0)} & {13-HideNSeek-Lava (C0)} & {14-CorridorBattle (C0)} \\
0-Room-Random & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Room-Dark & \cellcolor{green!20} 2.2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Room-Monster & \cellcolor{green!20} 7.7 & \cellcolor{green!20} 8.1 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Room-Trap & \cellcolor{green!20} 8.1 & \cellcolor{green!20} 8.9 & \cellcolor{green!20} 9.7 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Room-Ultimate & \cellcolor{green!20} 2.7 & \cellcolor{green!20} 4.6 & \cellcolor{green!20} 7.3 & \cellcolor{green!20} 8.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Corridor-R2 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 2.7 & \cellcolor{green!20} 4.0 & \cellcolor{green!20} 4.3 & \cellcolor{green!20} 3.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
6-Corridor-R3 & \cellcolor{green!20} 2.7 & \cellcolor{green!20} 2.8 & \cellcolor{green!20} 4.1 & \cellcolor{green!20} 4.4 & \cellcolor{green!20} 3.5 & \cellcolor{green!20} 4.7 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
7-KeyRoom & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.9 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 2.0 & \cellcolor{green!20} 2.1 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
8-KeyRoom-Dark & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 0.2 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} 0.1 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.5 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
9-River-Narrow & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
10-River-Monster & \cellcolor{green!20} 2.0 & \cellcolor{green!20} 2.1 & \cellcolor{green!20} 2.0 & \cellcolor{green!20} 1.9 & \cellcolor{green!20} 1.9 & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
11-River-Lava & \cellcolor{green!20} 1.7 & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.8 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.6 & \cellcolor{green!20} 1.3 & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.9 & \cellcolor{green!20} 0.9 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
12-HideNSeek & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 0.9 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 0.9 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
13-HideNSeek-Lava & \cellcolor{green!20} 1.1 & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.4 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.3 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} -0.1 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.4 & \cellcolor{green!20} 2.5 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
14-CorridorBattle & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.4 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} -0.0 & \cellcolor{white!20} 0.0 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.4 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} 0.1 & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

==> images/procgen/metrics/forgetting_tables.tex <==

\subfloat[IMPALA]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{green!1} -0.3 & \cellcolor{red!10} 2.5 & \cellcolor{red!4} 1.2 & \cellcolor{red!10} 2.6 & \cellcolor{red!7} 2.0 & \cellcolor{red!8} 2.0 & \cellcolor{red!6} 1.7 \\
1-Dodge.. & \cellcolor{red!24} 6.1 & \cellcolor{green!0} -0.1 & \cellcolor{red!20} 5.2 & \cellcolor{red!21} 5.4 & \cellcolor{red!24} 6.1 & \cellcolor{red!24} 6.2 & \cellcolor{red!19} 4.8 \\
2-Ninja & \cellcolor{green!1} -0.3 & \cellcolor{red!23} 6.0 & \cellcolor{green!4} -1.1 & \cellcolor{red!23} 5.9 & \cellcolor{red!20} 5.0 & \cellcolor{red!22} 5.7 & \cellcolor{red!14} 3.5 \\
3-Starp.. & \cellcolor{red!4} 1.2 & \cellcolor{red!3} 0.9 & \cellcolor{red!4} 1.2 & \cellcolor{green!15} -3.9 & \cellcolor{red!3} 0.8 & \cellcolor{red!4} 1.2 & \cellcolor{red!0} 0.2 \\
4-Bigfi.. & \cellcolor{red!7} 1.9 & \cellcolor{red!10} 2.6 & \cellcolor{red!8} 2.2 & \cellcolor{red!9} 2.4 & \cellcolor{green!7} -1.8 & \cellcolor{red!6} 1.7 & \cellcolor{red!5} 1.5 \\
5-Fruit.. & \cellcolor{red!26} 6.6 & \cellcolor{red!28} 7.0 & \cellcolor{red!28} 7.1 & \cellcolor{red!27} 6.8 & \cellcolor{red!28} 7.1 & \cellcolor{green!7} -1.8 & \cellcolor{red!21} 5.5 \\
\hline
Avg & \cellcolor{red!10} 2.5 & \cellcolor{red!12} 3.2 & \cellcolor{red!10} 2.6 & \cellcolor{red!12} 3.2 & \cellcolor{red!12} 3.2 & \cellcolor{red!10} 2.5 & \cellcolor{red!11} 2.9 \\
\hline
\end{tabular}
}
\subfloat[EWC]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!4} 1.2 & \cellcolor{red!4} 1.2 & \cellcolor{red!4} 1.1 & \cellcolor{red!5} 1.4 & \cellcolor{red!5} 1.3 & \cellcolor{red!5} 1.3 & \cellcolor{red!4} 1.2 \\
1-Dodge.. & \cellcolor{red!18} 4.7 & \cellcolor{red!14} 3.6 & \cellcolor{red!16} 4.1 & \cellcolor{red!13} 3.5 & \cellcolor{red!17} 4.4 & \cellcolor{red!19} 4.9 & \cellcolor{red!16} 4.2 \\
2-Ninja & \cellcolor{red!16} 4.0 & \cellcolor{red!16} 4.1 & \cellcolor{red!15} 3.9 & \cellcolor{red!17} 4.4 & \cellcolor{red!17} 4.3 & \cellcolor{red!16} 4.1 & \cellcolor{red!16} 4.1 \\
3-Starp.. & \cellcolor{green!2} -0.6 & \cellcolor{green!3} -0.8 & \cellcolor{green!2} -0.6 & \cellcolor{green!3} -0.8 & \cellcolor{green!3} -0.8 & \cellcolor{green!2} -0.6 & \cellcolor{green!2} -0.7 \\
4-Bigfi.. & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.1 & \cellcolor{red!1} 0.4 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.0 & \cellcolor{red!0} 0.2 \\
5-Fruit.. & \cellcolor{red!2} 0.7 & \cellcolor{red!2} 0.7 & \cellcolor{red!3} 0.8 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.3 & \cellcolor{red!2} 0.5 & \cellcolor{red!2} 0.6 \\
\hline
Avg & \cellcolor{red!6} 1.7 & \cellcolor{red!6} 1.5 & \cellcolor{red!6} 1.6 & \cellcolor{red!6} 1.5 & \cellcolor{red!6} 1.6 & \cellcolor{red!6} 1.7 & \cellcolor{red!6} 1.7 \\
\hline
\end{tabular}
}


\subfloat[Online EWC]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!9} 2.3 & \cellcolor{red!18} 4.7 & \cellcolor{red!7} 1.8 & \cellcolor{red!18} 4.6 & \cellcolor{red!15} 4.0 & \cellcolor{red!9} 2.4 & \cellcolor{red!13} 3.3 \\
1-Dodge.. & \cellcolor{red!24} 6.2 & \cellcolor{green!0} -0.0 & \cellcolor{red!20} 5.1 & \cellcolor{red!20} 5.2 & \cellcolor{red!23} 5.8 & \cellcolor{red!25} 6.5 & \cellcolor{red!19} 4.8 \\
2-Ninja & \cellcolor{red!12} 3.2 & \cellcolor{red!18} 4.7 & \cellcolor{red!5} 1.4 & \cellcolor{red!18} 4.6 & \cellcolor{red!17} 4.3 & \cellcolor{red!17} 4.4 & \cellcolor{red!15} 3.8 \\
3-Starp.. & \cellcolor{red!7} 2.0 & \cellcolor{red!1} 0.3 & \cellcolor{red!7} 2.0 & \cellcolor{green!4} -1.2 & \cellcolor{green!0} -0.2 & \cellcolor{red!7} 1.9 & \cellcolor{red!3} 0.8 \\
4-Bigfi.. & \cellcolor{green!0} -0.1 & \cellcolor{red!3} 0.9 & \cellcolor{green!0} -0.1 & \cellcolor{red!2} 0.6 & \cellcolor{red!0} 0.2 & \cellcolor{red!0} 0.1 & \cellcolor{red!1} 0.3 \\
5-Fruit.. & \cellcolor{green!0} -0.2 & \cellcolor{red!0} 0.2 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 & \cellcolor{red!0} 0.0 & \cellcolor{green!8} -2.1 & \cellcolor{green!1} -0.4 \\
\hline
Avg & \cellcolor{red!8} 2.2 & \cellcolor{red!7} 1.8 & \cellcolor{red!6} 1.7 & \cellcolor{red!9} 2.3 & \cellcolor{red!9} 2.3 & \cellcolor{red!8} 2.2 & \cellcolor{red!8} 2.2 \\
\hline
\end{tabular}
}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{green!0} -0.0 & \cellcolor{red!3} 0.8 & \cellcolor{red!7} 1.8 & \cellcolor{red!6} 1.6 & \cellcolor{red!7} 1.9 & \cellcolor{red!6} 1.5 & \cellcolor{red!5} 1.3 \\
1-Dodge.. & \cellcolor{red!12} 3.2 & \cellcolor{green!0} -0.0 & \cellcolor{green!0} -0.1 & \cellcolor{red!11} 2.8 & \cellcolor{red!11} 2.8 & \cellcolor{red!12} 3.1 & \cellcolor{red!7} 2.0 \\
2-Ninja & \cellcolor{red!1} 0.4 & \cellcolor{red!2} 0.6 & \cellcolor{red!1} 0.3 & \cellcolor{green!0} -0.0 & \cellcolor{red!6} 1.6 & \cellcolor{red!5} 1.5 & \cellcolor{red!2} 0.7 \\
3-Starp.. & \cellcolor{red!5} 1.4 & \cellcolor{green!0} -0.0 & \cellcolor{green!1} -0.3 & \cellcolor{green!2} -0.7 & \cellcolor{green!4} -1.1 & \cellcolor{red!3} 0.9 & \cellcolor{red!0} 0.0 \\
4-Bigfi.. & \cellcolor{green!3} -0.8 & \cellcolor{green!1} -0.4 & \cellcolor{red!1} 0.4 & \cellcolor{green!2} -0.5 & \cellcolor{green!1} -0.5 & \cellcolor{green!0} -0.1 & \cellcolor{green!1} -0.3 \\
5-Fruit.. & \cellcolor{green!4} -1.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.0 & \cellcolor{green!0} -0.1 & \cellcolor{green!0} -0.1 & \cellcolor{green!2} -0.7 & \cellcolor{green!1} -0.3 \\
\hline
Avg & \cellcolor{red!2} 0.5 & \cellcolor{red!0} 0.1 & \cellcolor{red!1} 0.3 & \cellcolor{red!2} 0.5 & \cellcolor{red!3} 0.8 & \cellcolor{red!4} 1.1 & \cellcolor{red!2} 0.6 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|llllll|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.1 & \cellcolor{red!0} 0.2 & \cellcolor{red!1} 0.3 & \cellcolor{red!1} 0.4 & \cellcolor{red!1} 0.3 & \cellcolor{red!0} 0.2 \\
1-Dodge.. & \cellcolor{green!2} -0.7 & \cellcolor{green!6} -1.7 & \cellcolor{green!4} -1.2 & \cellcolor{green!4} -1.0 & \cellcolor{green!3} -0.9 & \cellcolor{green!3} -0.9 & \cellcolor{green!4} -1.1 \\
2-Ninja & \cellcolor{green!0} -0.2 & \cellcolor{green!0} -0.1 & \cellcolor{green!2} -0.6 & \cellcolor{green!3} -0.9 & \cellcolor{green!2} -0.6 & \cellcolor{green!1} -0.4 & \cellcolor{green!1} -0.5 \\
3-Starp.. & \cellcolor{green!17} -4.3 & \cellcolor{green!17} -4.4 & \cellcolor{green!17} -4.4 & \cellcolor{green!26} -6.7 & \cellcolor{green!20} -5.1 & \cellcolor{green!18} -4.6 & \cellcolor{green!19} -4.9 \\
4-Bigfi.. & \cellcolor{green!9} -2.3 & \cellcolor{green!8} -2.2 & \cellcolor{green!8} -2.1 & \cellcolor{green!7} -2.0 & \cellcolor{green!16} -4.1 & \cellcolor{green!12} -3.1 & \cellcolor{green!10} -2.6 \\
5-Fruit.. & \cellcolor{green!11} -3.0 & \cellcolor{green!11} -2.9 & \cellcolor{green!11} -2.8 & \cellcolor{green!9} -2.4 & \cellcolor{green!8} -2.2 & \cellcolor{green!14} -3.6 & \cellcolor{green!11} -2.8 \\
\hline
Avg & \cellcolor{green!6} -1.7 & \cellcolor{green!7} -1.9 & \cellcolor{green!7} -1.8 & \cellcolor{green!8} -2.1 & \cellcolor{green!8} -2.1 & \cellcolor{green!8} -2.0 & \cellcolor{green!7} -1.9 \\
\hline
\end{tabular}
}



==> images/procgen/metrics/forgetting_tables_old.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} \\
\hline
0-Climb... & \cellcolor{white!20} -- & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 \\
1-Dodge... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 \\
2-Ninja & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 2.5 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 2.6 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 2.8 & \cellcolor{red!20} 2.9 & \cellcolor{red!20} 2.6 \\
3-Starp... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.9 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.9 & \cellcolor{green!20} -0.4 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.7 \\
4-Bigfi... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.9 & \cellcolor{red!20} 0.4 & \cellcolor{green!20} -0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.0 & \cellcolor{red!20} 0.2 \\
5-Fruit... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -1.2 & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -0.9 & \cellcolor{green!20} -0.8 & \cellcolor{red!20} 0.1 \\
\hline
\end{tabular}
}

\subfloat[EWC]{ 
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} \\
\hline
0-Climb... & \cellcolor{white!20} -- & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 \\
1-Dodge... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.8 \\
2-Ninja & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.2 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.0 \\
3-Starp... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.5 \\
4-Bigfi... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -0.5 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.9 & \cellcolor{green!20} -0.1 \\
5-Fruit... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 \\
\hline
\end{tabular}
}

\subfloat[ONLINE EWC]{ 
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} \\
\hline
0-Climb... & \cellcolor{white!20} -- & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.5 \\
1-Dodge... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 0.8 & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.7 \\
2-Ninja & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 1.8 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.5 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 1.9 & \cellcolor{red!20} 2.0 & \cellcolor{red!20} 1.6 \\
3-Starp... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.6 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.9 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 \\
4-Bigfi... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.8 & \cellcolor{green!20} -2.0 & \cellcolor{red!20} 1.1 & \cellcolor{green!20} -1.3 & \cellcolor{red!20} 1.1 & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -1.0 \\
5-Fruit... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.4 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.1 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.1 \\
\hline
\end{tabular}
}

\subfloat[P\&C]{ 
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} \\
\hline
0-Climb... & \cellcolor{white!20} -- & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 \\
1-Dodge... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.4 \\
2-Ninja & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 0.9 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.7 & \cellcolor{red!20} 0.6 \\
3-Starp... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.4 & \cellcolor{green!20} -0.2 & \cellcolor{red!20} 0.2 & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.3 \\
4-Bigfi... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.8 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.8 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 0.8 & \cellcolor{green!20} -0.1 \\
5-Fruit... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.1 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.1 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|Hlllllllllll|}
\hline
{} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} & {0-Climb...} & {1-Dodge...} & {2-Ninja} & {3-Starp...} & {4-Bigfi...} & {5-Fruit...} \\
\hline
0-Climb... & \cellcolor{white!20} -- & \cellcolor{green!20} -0.0 & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.0 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.1 \\
1-Dodge... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.0 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.3 \\
2-Ninja & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.5 & \cellcolor{green!20} -0.1 & \cellcolor{red!20} 0.0 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.4 & \cellcolor{green!20} -0.0 & \cellcolor{red!20} 0.1 & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.3 \\
3-Starp... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{green!20} -0.2 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.5 & \cellcolor{green!20} -0.6 & \cellcolor{green!20} -0.7 & \cellcolor{green!20} -2.1 & \cellcolor{green!20} -1.9 & \cellcolor{green!20} -1.9 \\
4-Bigfi... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.6 & \cellcolor{red!20} 1.0 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.4 & \cellcolor{red!20} 1.1 & \cellcolor{red!20} 1.3 & \cellcolor{red!20} 1.6 \\
5-Fruit... & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{red!20} 0.3 & \cellcolor{red!20} 0.2 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.5 & \cellcolor{red!20} 0.4 & \cellcolor{red!20} 0.6 \\
\hline
\end{tabular}
}

==> images/procgen/metrics/transfer_tables.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
{} & {0-Climb..} & {1-Dodge..} & {2-Ninja} & {3-Starp..} & {4-Bigfi..} & {5-Fruit..} & {Avg} \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.4 \\
2-Ninja & \cellcolor{green!16} 4.0 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.9 \\
3-Starp.. & \cellcolor{red!0} -0.2 & \cellcolor{green!8} 2.2 & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
4-Bigfi.. & \cellcolor{green!22} 5.7 & \cellcolor{red!4} -1.1 & \cellcolor{red!0} -0.0 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
5-Fruit.. & \cellcolor{green!4} 1.1 & \cellcolor{green!1} 0.4 & \cellcolor{green!0} 0.2 & \cellcolor{green!1} 0.4 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!1} 0.5 \\
\hline
Avg & \cellcolor{green!8} 2.1 & \cellcolor{green!1} 0.3 & \cellcolor{green!0} 0.2 & \cellcolor{red!1} -0.4 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
{} & {0-Climb..} & {1-Dodge..} & {2-Ninja} & {3-Starp..} & {4-Bigfi..} & {5-Fruit..} & {Avg} \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
2-Ninja & \cellcolor{red!5} -1.4 & \cellcolor{red!16} -4.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!11} -2.8 \\
3-Starp.. & \cellcolor{red!1} -0.3 & \cellcolor{green!24} 6.2 & \cellcolor{green!8} 2.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!10} 2.7 \\
4-Bigfi.. & \cellcolor{red!1} -0.3 & \cellcolor{red!12} -3.1 & \cellcolor{red!4} -1.1 & \cellcolor{red!11} -2.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!7} -1.8 \\
5-Fruit.. & \cellcolor{green!2} 0.6 & \cellcolor{red!7} -1.8 & \cellcolor{red!0} -0.2 & \cellcolor{red!3} -1.0 & \cellcolor{red!2} -0.7 & \cellcolor{red!0} -- & \cellcolor{red!2} -0.6 \\
\hline
Avg & \cellcolor{red!1} -0.3 & \cellcolor{red!2} -0.7 & \cellcolor{green!1} 0.3 & \cellcolor{red!7} -1.9 & \cellcolor{red!2} -0.7 & \cellcolor{red!0} -- & \cellcolor{red!2} -0.5 \\
\hline
\end{tabular}
}




\subfloat[Online EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
{} & {0-Climb..} & {1-Dodge..} & {2-Ninja} & {3-Starp..} & {4-Bigfi..} & {5-Fruit..} & {Avg} \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
2-Ninja & \cellcolor{green!5} 1.4 & \cellcolor{red!8} -2.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.3 \\
3-Starp.. & \cellcolor{red!3} -0.8 & \cellcolor{green!12} 3.2 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!3} 0.8 \\
4-Bigfi.. & \cellcolor{green!16} 4.2 & \cellcolor{red!2} -0.6 & \cellcolor{green!12} 3.1 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!6} 1.7 \\
5-Fruit.. & \cellcolor{green!3} 0.9 & \cellcolor{red!5} -1.3 & \cellcolor{green!3} 1.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
Avg & \cellcolor{green!4} 1.1 & \cellcolor{red!0} -0.2 & \cellcolor{green!5} 1.3 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{green!2} 0.6 \\
\hline
\end{tabular}
}
\hspace{3em}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
{} & {0-Climb..} & {1-Dodge..} & {2-Ninja} & {3-Starp..} & {4-Bigfi..} & {5-Fruit..} & {Avg} \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
2-Ninja & \cellcolor{green!7} 1.8 & \cellcolor{green!6} 1.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!6} 1.7 \\
3-Starp.. & \cellcolor{red!8} -2.1 & \cellcolor{red!2} -0.5 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!3} -0.9 \\
4-Bigfi.. & \cellcolor{red!1} -0.3 & \cellcolor{red!6} -1.5 & \cellcolor{red!6} -1.7 & \cellcolor{red!7} -1.9 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!5} -1.4 \\
5-Fruit.. & \cellcolor{green!5} 1.5 & \cellcolor{green!7} 1.9 & \cellcolor{green!6} 1.7 & \cellcolor{green!5} 1.4 & \cellcolor{green!7} 1.8 & \cellcolor{red!0} -- & \cellcolor{green!6} 1.7 \\
\hline
Avg & \cellcolor{green!0} 0.2 & \cellcolor{green!1} 0.4 & \cellcolor{red!0} -0.0 & \cellcolor{red!1} -0.3 & \cellcolor{green!7} 1.8 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
\hline
\end{tabular}
}




\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
{} & {0-Climb..} & {1-Dodge..} & {2-Ninja} & {3-Starp..} & {4-Bigfi..} & {5-Fruit..} & {Avg} \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.2 \\
2-Ninja & \cellcolor{green!14} 3.6 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 1.8 \\
3-Starp.. & \cellcolor{red!0} -0.1 & \cellcolor{green!5} 1.3 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!1} 0.5 \\
4-Bigfi.. & \cellcolor{green!19} 4.9 & \cellcolor{green!1} 0.5 & \cellcolor{green!7} 1.9 & \cellcolor{green!3} 0.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!7} 2.0 \\
5-Fruit.. & \cellcolor{green!4} 1.2 & \cellcolor{red!2} -0.7 & \cellcolor{red!1} -0.4 & \cellcolor{red!4} -1.1 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{red!1} -0.5 \\
\hline
Avg & \cellcolor{green!7} 2.0 & \cellcolor{green!1} 0.3 & \cellcolor{green!2} 0.6 & \cellcolor{red!0} -0.2 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -- & \cellcolor{green!2} 0.7 \\
\hline
\end{tabular}
}

==> images/procgen/metrics/transfer_tables_isolated.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} 0.0 \\
2-Ninja & \cellcolor{green!12} 3.0 & \cellcolor{red!16} -4.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!2} -0.6 \\
3-Starp.. & \cellcolor{red!0} -0.0 & \cellcolor{green!1} 0.3 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
4-Bigfi.. & \cellcolor{green!4} 1.1 & \cellcolor{red!8} -2.0 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
5-Fruit.. & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -0.1 & \cellcolor{green!1} 0.3 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
Avg & \cellcolor{green!3} 0.8 & \cellcolor{red!6} -1.5 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
\hline
\end{tabular}
}
\subfloat[EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!1} -0.4 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.4 \\
2-Ninja & \cellcolor{green!9} 2.3 & \cellcolor{red!13} -3.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.5 \\
3-Starp.. & \cellcolor{red!5} -1.3 & \cellcolor{green!13} 3.5 & \cellcolor{red!12} -3.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!1} -0.3 \\
4-Bigfi.. & \cellcolor{green!15} 3.8 & \cellcolor{red!17} -4.3 & \cellcolor{green!6} 1.6 & \cellcolor{red!6} -1.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
5-Fruit.. & \cellcolor{red!0} -0.1 & \cellcolor{red!8} -2.1 & \cellcolor{green!6} 1.6 & \cellcolor{red!1} -0.4 & \cellcolor{green!1} 0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
\hline
Avg & \cellcolor{green!3} 0.9 & \cellcolor{red!6} -1.5 & \cellcolor{green!0} 0.0 & \cellcolor{red!3} -1.0 & \cellcolor{green!1} 0.5 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
\hline
\end{tabular}
}


\subfloat[Online EWC]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!2} -0.6 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!2} -0.6 \\
2-Ninja & \cellcolor{green!17} 4.5 & \cellcolor{red!17} -4.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
3-Starp.. & \cellcolor{red!2} -0.7 & \cellcolor{green!8} 2.2 & \cellcolor{red!8} -2.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
4-Bigfi.. & \cellcolor{green!7} 1.8 & \cellcolor{red!10} -2.7 & \cellcolor{green!4} 1.1 & \cellcolor{red!3} -0.8 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
5-Fruit.. & \cellcolor{green!1} 0.3 & \cellcolor{red!1} -0.5 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
Avg & \cellcolor{green!4} 1.1 & \cellcolor{red!5} -1.3 & \cellcolor{red!0} -0.2 & \cellcolor{red!1} -0.5 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
\hline
\end{tabular}
}
\subfloat[P\&C]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!2} -0.7 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!2} -0.7 \\
2-Ninja & \cellcolor{green!6} 1.6 & \cellcolor{red!1} -0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!2} 0.7 \\
3-Starp.. & \cellcolor{red!3} -0.9 & \cellcolor{green!3} 0.8 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
4-Bigfi.. & \cellcolor{green!5} 1.4 & \cellcolor{red!2} -0.7 & \cellcolor{red!2} -0.7 & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
5-Fruit.. & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -0.1 & \cellcolor{red!0} -0.2 & \cellcolor{green!0} 0.1 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.0 \\
\hline
Avg & \cellcolor{green!1} 0.3 & \cellcolor{red!0} -0.1 & \cellcolor{red!1} -0.3 & \cellcolor{green!0} 0.2 & \cellcolor{green!0} 0.2 & \cellcolor{red!0} -- & \cellcolor{green!0} 0.1 \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllH|l|}
\hline
 & 0-Climb.. & 1-Dodge.. & 2-Ninja & 3-Starp.. & 4-Bigfi.. & 5-Fruit.. & Avg \\
\hline
0-Climb.. & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- \\
1-Dodge.. & \cellcolor{red!0} -0.2 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.2 \\
2-Ninja & \cellcolor{green!12} 3.2 & \cellcolor{red!13} -3.3 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
3-Starp.. & \cellcolor{red!0} -0.1 & \cellcolor{green!0} 0.1 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
4-Bigfi.. & \cellcolor{green!2} 0.6 & \cellcolor{red!4} -1.2 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
5-Fruit.. & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.0 \\
\hline
Avg & \cellcolor{green!2} 0.7 & \cellcolor{red!4} -1.1 & \cellcolor{red!0} -0.0 & \cellcolor{red!0} -0.0 & \cellcolor{green!0} 0.0 & \cellcolor{red!0} -- & \cellcolor{red!0} -0.1 \\
\hline
\end{tabular}
}


==> images/procgen/metrics/transfer_tables_old.tex <==
\subfloat[IMPALA]{ 
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-Climber (C0)} & {1-Dodgeball (C0)} & {2-Ninja (C0)} & {3-Starpilot (C0)} & {4-Bigfish (C0)} & {5-Fruitbot (C0)} \\
\hline
0-Climber & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Dodgeball & \cellcolor{red!20} -0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Ninja & \cellcolor{green!20} 1.8 & \cellcolor{red!20} -0.1 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Starpilot & \cellcolor{red!20} -0.1 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 0.2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Bigfish & \cellcolor{green!20} 4.1 & \cellcolor{red!20} -0.8 & \cellcolor{red!20} -0.0 & \cellcolor{red!20} -1.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Fruitbot & \cellcolor{green!20} 0.8 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 0.0 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[EWC]{ 
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-Climber (C0)} & {1-Dodgeball (C0)} & {2-Ninja (C0)} & {3-Starpilot (C0)} & {4-Bigfish (C0)} & {5-Fruitbot (C0)} \\
\hline
0-Climber & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Dodgeball & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Ninja & \cellcolor{red!20} -0.8 & \cellcolor{red!20} -2.5 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Starpilot & \cellcolor{red!20} -0.1 & \cellcolor{green!20} 1.2 & \cellcolor{green!20} 0.4 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Bigfish & \cellcolor{red!20} -0.6 & \cellcolor{red!20} -5.4 & \cellcolor{red!20} -1.9 & \cellcolor{red!20} -5.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Fruitbot & \cellcolor{green!20} 0.2 & \cellcolor{red!20} -0.5 & \cellcolor{red!20} -0.1 & \cellcolor{red!20} -0.3 & \cellcolor{red!20} -0.2 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[Online EWC]{ 
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-Climber (C0)} & {1-Dodgeball (C0)} & {2-Ninja (C0)} & {3-Starpilot (C0)} & {4-Bigfish (C0)} & {5-Fruitbot (C0)} \\
\hline
0-Climber & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Dodgeball & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Ninja & \cellcolor{green!20} 0.6 & \cellcolor{red!20} -0.8 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Starpilot & \cellcolor{red!20} -0.3 & \cellcolor{green!20} 1.0 & \cellcolor{red!20} -0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Bigfish & \cellcolor{green!20} 3.4 & \cellcolor{red!20} -0.5 & \cellcolor{green!20} 2.6 & \cellcolor{green!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Fruitbot & \cellcolor{green!20} 0.2 & \cellcolor{red!20} -0.3 & \cellcolor{green!20} 0.2 & \cellcolor{green!20} 0.0 & \cellcolor{red!20} -0.0 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[P\&C]{ 
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-Climber (C0)} & {1-Dodgeball (C0)} & {2-Ninja (C0)} & {3-Starpilot (C0)} & {4-Bigfish (C0)} & {5-Fruitbot (C0)} \\
\hline
0-Climber & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Dodgeball & \cellcolor{white!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Ninja & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.9 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Starpilot & \cellcolor{red!20} -0.6 & \cellcolor{red!20} -0.2 & \cellcolor{red!20} -0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Bigfish & \cellcolor{red!20} -0.3 & \cellcolor{red!20} -1.7 & \cellcolor{red!20} -1.9 & \cellcolor{red!20} -2.2 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Fruitbot & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.7 & \cellcolor{green!20} 0.6 & \cellcolor{green!20} 0.5 & \cellcolor{green!20} 0.7 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}

\subfloat[CLEAR]{ 
 \begin{tabular}{|l|lllllH|}
\hline
{} & {0-Climber (C0)} & {1-Dodgeball (C0)} & {2-Ninja (C0)} & {3-Starpilot (C0)} & {4-Bigfish (C0)} & {5-Fruitbot (C0)} \\
\hline
0-Climber & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
1-Dodgeball & \cellcolor{green!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
2-Ninja & \cellcolor{green!20} 1.5 & \cellcolor{green!20} 0.0 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
3-Starpilot & \cellcolor{red!20} -0.1 & \cellcolor{green!20} 1.0 & \cellcolor{green!20} 0.3 & \cellcolor{white!20} -- & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
4-Bigfish & \cellcolor{green!20} 3.7 & \cellcolor{green!20} 0.3 & \cellcolor{green!20} 1.4 & \cellcolor{green!20} 0.6 & \cellcolor{white!20} -- & \cellcolor{white!20} -- \\
5-Fruitbot & \cellcolor{green!20} 0.5 & \cellcolor{red!20} -0.3 & \cellcolor{red!20} -0.2 & \cellcolor{red!20} -0.5 & \cellcolor{red!20} -0.6 & \cellcolor{white!20} -- \\
\hline
\end{tabular}
}


==> metric_tables_old.tex <==
\clearpage
\section{Metrics}
\label{section:metrics_tables_old}

Recall that in all cases, each table represents how much training on the task in each column impacts the performance of the task in each row. 
% \todo{fix spacing}

\subsection{Atari Metrics: (Max) Forgetting}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/atari/metrics/forgetting_tables}
\vspace{2em}
\caption{Atari Forgetting metrics. We can see that forgetting across the board is quite high, though mitigated by both EWC and CLEAR.}
\label{tab:atari_forgetting}
\end{table}

\clearpage

\subsection{Atari Metrics: Transfer}
\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/atari/metrics/transfer_tables}
\vspace{2em}
\caption{Atari Transfer metrics. Note that overall there is little forward transfer observed; this is expected because the tasks bear little similarity.}
\label{tab:atari_transfer}
\end{table}

\clearpage

\subsection{Procgen Metrics: (Max) Forgetting}
\label{sec:procgen_forgetting}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/procgen/metrics/forgetting_tables}
\vspace{2em}
\caption{Procgen Forgetting metrics}
\label{tab:procgen_forgetting}
\end{table}

\subsection{Procgen Metrics: Transfer}
\label{sec:procgen_transfer}

% \begin{table}[H]
% \setlength\tabcolsep{2pt} % default value: 6pt
% \tiny
% \input{images/procgen/metrics/transfer_tables}
% \vspace{2em}
% \caption{Procgen cumulative Transfer metrics}
% \label{tab:procgen_transfer}
% \end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/procgen/metrics/transfer_tables_isolated}
\vspace{2em}
\caption{Procgen Transfer metrics}
\label{tab:procgen_transfer}
\end{table}

\clearpage

\subsection{MiniHack Metrics: (Max) Forgetting}
\label{sec:minihack_forgetting}

\begin{table}[ht]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/minihack/metrics/forgetting_tables_10x}
\vspace{2em}
\label{tab:minihack_forgetting}
\end{table}

\clearpage
\subsection{MiniHack Metrics: Transfer}
\label{sec:minihack_transfer}

% \begin{table}[ht]
% \setlength\tabcolsep{2pt} % default value: 6pt
% \tiny
% \input{images/minihack/metrics/transfer_tables_10x}
% \vspace{2em}
% \caption{MiniHack cumulative Transfer metrics. 
% }
% \label{tab:minihack_transfer}
% \end{table}

\begin{table}[ht]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/minihack/metrics/transfer_tables_10x_isolated}
\vspace{2em}
\caption{MiniHack Transfer metrics. 
}
\label{tab:minihack_transfer}
\end{table}

\clearpage

\subsection{CHORES Metrics: (Max) Forgetting}
\label{sec:chores_forgetting}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_envs_forgetting}
\vspace{2em}
\caption{CHORES: Mem-VaryRoom (Max) Forgetting metrics}
\label{tab:chores_vary_env_forgetting}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_tasks_forgetting}
\vspace{2em}
\caption{CHORES: Mem-VaryTasks (Max) Forgetting metrics}
\label{tab:chores_vary_tasks_forgetting}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_objects_forgetting}
\vspace{2em}
\caption{CHORES: Mem-VaryObjects (Max) Forgetting metrics}
\label{tab:chores_vary_objects_forgetting}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/multi_traj_forgetting}
\vspace{2em}
\caption{CHORES: Gen-MultiTraj (Max) Forgetting metrics}
\label{tab:chores_multi_traj_forgetting}
\end{table}

\clearpage

\subsection{CHORES Metrics: Transfer}
\label{sec:chores_transfer}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_envs_transfer}
\vspace{2em}
\caption{CHORES: Mem-VaryRoom Transfer metrics}
\label{tab:chores_vary_env_transfer}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_tasks_transfer}
\vspace{2em}
\caption{CHORES: Mem-VaryTasks Transfer metrics}
\label{tab:chores_vary_tasks_transfer}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/vary_objects_transfer}
\vspace{2em}
\caption{CHORES: Mem-VaryObjects Transfer metrics}
\label{tab:chores_vary_objects_transfer}
\end{table}

\begin{table}[H]
\tablemarginhack
\setlength\tabcolsep{2pt} % default value: 6pt
\tiny
\input{images/chores/metrics/multi_traj_transfer}
\vspace{2em}
\caption{CHORES: Gen-MultiTraj Transfer metrics}
\label{tab:chores_multi_traj_transfer}
\end{table}
